A Pattern Logic for Automata with Outputs

We introduce a logic to express structural properties of automata with string inputs and, possibly, outputs in some monoid. In this logic, the set of predicates talking about the output values is parametric, and we provide sufficient conditions on the predicates under which the model-checking problem is decidable. We then consider three particular automata models (finite automata, transducers and automata weighted by integers -- sum-automata --) and instantiate the generic logic for each of them. We give tight complexity results for the three logics and the model-checking problem, depending on whether the formula is fixed or not. We study the expressiveness of our logics by expressing classical structural patterns characterising for instance finite ambiguity and polynomial ambiguity in the case of finite automata, determinisability and finite-valuedness in the case of transducers and sum-automata. Consequently to our complexity results, we directly obtain that these classical properties can be decided in PTIME.

==> app-extensions.tex <==
\section{Extensions}

\subsection{State colouring}

In the model of automata with outputs, states can receive a subset of
colours in $\{\init,\final\}$, which can be identified through the
unary predicates $\init(p)$ and $\final(p)$ in the logic $\logic$. All
our complexity results carry over to any automata with outputs
whose states can get subsets of colours within a
fixed but arbitrary finite set of colours $K$, and to the logic
$\logic$ extended with unary predicates $c(q)$, $c\in K$. 

This might be useful for instance to express properties of disjoint
unions of automata, where two different colours are used to distinguish
states of the first automaton from states of the other one. As
an example, assume we want to check, given two sum-automata $S_1,S_2$,
whether there exists an input word $u$ such that $S_1(u)\cap
S_2(u)\neq \varnothing$. This property holds iff the disjoint union
$S_1\uplus S_2$ (where states of $S_i$ are coloured by $c_i$) satisfy
the formula:
$$
\exists \pi_1:p_1\xrightarrow{u\mid v} q_1,\exists
\pi_2:p_2\xrightarrow{u\mid v}
q_2,\bigwedge_{i=1}^2 \init(p_i)\wedge \final(q_i)\wedge
c_i(p_i)\wedge c_i(q_i)
 $$


\subsection{Universal quantification over states}

The logic $\logic$ is purely existential. However simple properties
such as whether all states of an automaton are reachable from an
initial state are not directly expressible in $\logic$. We define
therefore the extension denoted $\forall^* Q\logic[\O]$ to be all
formulas of the form $\forall q_1\dots \forall q_m \phi$ where
$\phi\in \logic[\O]$. In $\forall^* Q\logic[\O]$, the previous
property is expressible by 
$$
\forall q\exists \pi:q_0\xrightarrow{u\mid v} q,\init(q_0)
$$
The complexity of model-checking does not change (for all the
particular instances of the logic we have considered: finite automata,
transducers and sum-automata) if we allow for universal state
quantification. Indeed, if the formula is not fixed, it suffices to
iterate over all $m$-tuples of states and call a \textsc{PSPace}
algorithm over the automaton where these states have been marked
(thanks to some colouring, as seen previously), this remains
\textsc{PSpace}. If the formula is fixed, then
there is only a polynomial number of $m$-tuples of states.

\begin{theorem}
    Over finite automata, the model-checking problem of formulas in 
    $\forall^* Q\logic_{Reg}$ is \textsc{PSPace-c}, and \textsc{PTime}
    if the formula is fixed. 


    Over transducers, the model-checking problem of formulas in 
    $\forall^* Q\logic_{Trans}$ is \textsc{PSPace-c}, and \textsc{PTime}
    if the formula is fixed. 


    Over finite automata, the model-checking problem of formulas in 
    $\forall^* Q\logic_{Sum}$ is \textsc{PSPace-c}, \textsc{NP-c}
    if the formula is fixed, and \textsc{PTime} if additionally the
    values of the automaton are unary encoded. The fragment
    $\forall^*Q\logic^+[\neq]$ has \textsc{PTime} model-checking
    problem for a fixed formula. 
\end{theorem}


%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:


==> app-logic.tex <==
\section{Model-checking algorithms -- Section \ref{sec:MC}}


\subsection{An intermediate syntax for formulas}

In the pattern logic, we have four types of variables (runs, states, inputs and outputs).
While this is appealing for succinctness and readability reasons, it is less easy to deal with at an algorithmic level.
Therefore, we introduce here another syntax, called paths formulas, in which there is a single type of variables: path variables.
We then show that the two logics are equivalent in the sense that satisfiability by any automaton with output is preserved. 


% ----------------------------------------------------------------------- %


\begin{definition}
	Let $X$ a set of path variables and $\O$ a set of output predicates.
	A \emph{path formula} $\varphi$ over $\O$ is a term generated by the following grammar:
	$$
		\begin{array}{lcll}
			\text{path formula} & \varphi \Coloneqq &
				\varphi \land \varphi \mid
				\varphi \lor \varphi \mid
				\lnot \varphi \mid
		\smallskip\\
			\text{input constraints} &&
				\pi_1 \prefix_I \pi_2 \mid
				\pi \in_I L \mid
				\pi_1 \leq^\text{len}_I \pi_2 \mid
		\smallskip\\
			\text{state constraints} &&
				\init(\pi^d) \mid
				\final(\pi^d) \mid
				\pi_1^{d_1} =_Q \pi_2^{d_2} \mid 
		\smallskip\\ 
			\text{path constraints} &&
				\pi_1 =_P \pi_2
		\smallskip\\
			\text{output constraints} &&
				p(t_1,\dots,t_{\alpha(p)})
				%& \forall p\in\O
		\end{array}
	$$
	where $\pi,\pi_1,\pi_2\in X$, $d,d_1,d_2\in\{\first,\last\}$
	$t_1,\dots,t_n\in \text{Terms}(X,\oplus,\zero)$,
	$p \in \O$ of arity $\alpha(p)$ and
	$L$ ranges over regular languages over $\Lambda$.
	We denote by $\logic_P(\O)$ the set of paths formulas over
        $\O$, and by $\logic_P^+(\O)$ its fragment where output
        predicates does not occur under an odd number of negations. 
\end{definition}

We introduce usual syntactic sugar:
$(\pi =_I \pi') \new \pi\prefix_I \pi' \land  \pi'\prefix_I \pi$,
$(\pi=^\text{len}_I \pi') \new (\pi\leq^\text{len}_I \pi')\land (\pi'\leq^\text{len}_I \pi)$,
$(\pi<^\text{len}_I \pi') \new \lnot (\pi'\leq^\text{len}_I \pi)$,

Informally, paths formulas only speak about the runs of an automaton
with output, the input constraints speak about properties of their
inputs, the state contraints about properties of their starting and
ending states, and $\O$ about properties of their outputs.
The semantics of such a formula is then, on an automaton with output
$A$, valuations of path variables into runs in $\paths(A)$. 


Formally, we first fix some monoid $\M = (D,\oplus_\M,\zero_\M)$ together with an interpretation ${p}^\M$ of each output predicate $p \in \O$.
Let $A \in \trs(\M)$ be an automaton with output. Given a valuation
$\nu\colon X\rightarrow \paths(A)$, the interpretation $t^{\nu,\M}\in
D$ of terms $t\in\text{Terms}(X,\oplus,\zero)$ is inductively defined
by $(t_1\oplus t_2)^{\nu,\M} = t_1^{\nu,\M}\oplus t_2^{\nu,\M}$,
$\zero^{\nu,\M} = \zero_\M$ and $\pi^{\nu,\M} = \out(\nu(\pi))\in D$. Then a formula $\varphi \in
\logic_P(\O)$ is interpreted in $A= (Q, I, F, \Delta, \gamma)$ as a
set of valuations denoted $\sem{\varphi}_A\subseteq\paths(A)^{X}$ defined as follows.
$$
	\begin{array}{l}
		\sem{\init(\pi^d)}_A = \{ \nu \  \mid \nu(\pi)^d \in I \}
	\smallskip\\
		\sem{\pi_1^{d_1} =_Q \pi_2^{d_2}}_A = \{ \nu \  \mid \nu(\pi_1)^{d_1} = \nu(\pi_2)^{d_2} \}
	\smallskip\\
		\sem{\final(\pi^d)}_A = \{ \nu \  \mid \nu(\pi)^d \in F \}
	\smallskip\\
		\sem{\lnot\varphi}_A = \paths(A)^{X} \setminus \sem{\varphi}_A
	\smallskip\\
		\sem{\varphi_1 \land \varphi_2}_A = \sem{\varphi_1}_A \cap \sem{\varphi_2}_A
	\smallskip\\
		\sem{\varphi_1 \lor \varphi_2}_A = \sem{\varphi_1}_A \cup \sem{\varphi_2}_A
	\smallskip\\
		\sem{\pi_1 \prefix_I \pi_2}_A = \{ \nu \  \mid \inp(\nu(\pi_1)) \prefix \inp(\nu(\pi_2)) \}
	\smallskip\\
		\sem{\pi_1 =_P \pi_2}_A = \{ \nu \  \mid \nu(\pi_1) = \nu(\pi_2) \}
	\smallskip\\
		\sem{\pi_1 \leq^{len}_I \pi_2}_A = \{ \nu \  \mid |\inp(\nu(\pi_1))| \leq |\inp(\nu(\pi_2))| \}
	\smallskip\\
		\sem{\pi \in_I L}_A = \{ \nu \  \mid \inp(\nu(\pi)) \in L \}
	\smallskip\\
		\sem{p(t_1,\dots,t_{\alpha(p)})}_A = \{ \nu \  \mid (t_1^{\nu, \M},\dots,t_{\alpha(p)}^{\nu, \M}) \in p^\M\}
	\end{array}
$$
A path formula $\varphi$ is said to be satisfiable over $A$ if
$\sem{\varphi}_A \neq \varnothing$. The path logic and the pattern
logic are equivalent in the following precise sense. 


% ----------------------------------------------------------------------- %


\begin{lemma} \label{lem:translate}
	For all pattern formulas $\varphi \in \logic(\O)$, 
        (resp. $\varphi\in\logic^+(\O)$), one can construct in linear
        time a path formula $\psi \in \logic_P(\O\cup\{=_O\})$
        (resp. $\psi\in\logic_P^+(\O\cup \{=_O\})$) such
        that the following hold:
	\begin{enumerate}
	\item
		$\Var_P(\varphi) = \Var(\psi)$
	\item
		for all monoid $\M = (D,\oplus_\M,\zero_\M)$,
		all interpretation $p^\M \in D^{\alpha(p)}$ for each $p \in \O$,
		all automata with output $A \in \trs(\M)$,  we have $A\models \varphi$ iff $A\models \psi$
		\item there is a surjective mapping from the valuations (in $A$)  satisfying $\psi$ to the valuations satisfying $\varphi$. 
	\end{enumerate}
	In addition, if $\varphi$ does not contain twice the same output variable in its prefix, then $\psi \in \logic_P(\O)$.
\end{lemma}

\begin{proof}
	Assume that $\varphi$ is of the form:
	$$
	\exists \pi_1:p_1\xrightarrow{u_1\mid
		v_1} q_1\ldots \exists \pi_n:p_n\xrightarrow{u_n\mid
		v_n} q_n\cdot \mathcal{C}
	$$
	In a first step, we rename the $j$-th occurrences, $j>1$, of any
	state, input and output variables so that eventually, all these
	variables are pairwise different in the prefix. This can be easily
	done in linear-time modulo adding some equality constraints to
	$\mathcal{C}$. For instance, if we have $p_i = p_j$, $i<j$, we use
	a fresh variable name $p$ and replace $p_j$ by $p$ in the prefix
	$\exists \pi_1\dots \exists \pi_n$, and add the constraint $p =
	p_i$ to $\mathcal{C}$. We do the same for the other types of
	variables. Note that it is not necessary to do it for the path
	variables $\pi_i$, since by definition of pattern formulas, they
	are assumed to occur only once in the prefix. 
	
	
	We end up with a formula of the form 
	$$
	\varphi' \equiv \exists \pi_1:p'_1\xrightarrow{u'_1\mid
		v'_1} q'_1\ldots \exists \pi_n:p'_n\xrightarrow{u'_n\mid
		v'_n} q'_n\cdot \mathcal{C'}
	$$
	where all the variables occur once in the prefix,
	together with a mapping $f$ from the new variables to
	the old ones. We also assume that $f$ is the identify
	on the path variables. In our previous example, we would have
	$f(p) = p_j$ for instance. 
	
	Then, $\varphi'$ and $\varphi$ are equivalent in the
	following sense: over an automaton with output, for all 
	valuations $\nu$ satisfying $\varphi$, $\nu\circ
	f$ satisfies $\varphi'$. Conversely, for all
	valuations $\nu'$ satisfying $\varphi'$, the valuation 
	$\nu'$ restricted to the variables of $\varphi$
	satisfies $\varphi$. Hence, it is possible to recover
	the models of $\varphi$ from the models of $\varphi'$,
	and conversely. 
	
	Now, note that in $\varphi'$, there is a functional
	dependency between the state, input and output
	variables, and the path variables. This dependency is
	formalised through three functions $f_Q, f_I, f_O$
	from respectively,
	$\{p'_1,\dots,p'_n,q'_1,\dots,q'_n\}$ to
	$\{\pi_1,\dots,\pi_n\}$, $\{ u'_1,\dots,u'_n\}$ to 
	$\{\pi_1,\dots,\pi_n\}$, and from $\{
	v'_1,\dots,v'_n\}$ to $\{\pi_1,\dots,\pi_n\}$. 
	
	Then, $\psi$ is obtained by applying the following
	transformations on $\mathcal{C}$:
	\begin{itemize}
	\item
		Any atom $u\prefix u'$ is replaced by $f_I(u)\prefix_I f_I(u')$.
		Any atom $u\in L$ by $f_I(u)\in_I L$.
		Any atom $|u|\leq |u'|$ by $f_I(u) \leq_I^\text{len} f_I(u')$.
	\item
		Any atom $p(t_1,\dots,t_k)$ is replaced by $p(t'_1,\dots,t'_k)$ where $t'_i$ is obtained by substituting any variable $v$ in $t_i$ by $f_O(v)$.
	\item
		Any atom $\init(q)$ is replaced by $\init(f_Q(q)^\first)$ if there exists a binding $\exists \pi \colon q\xrightarrow{u\mid v} q'$ in $\varphi'$ otherwise $\init(q)$ is replaced by $\init(f_Q(q)^\last)$ and there exists a binding $\exists \pi \colon q'\xrightarrow{u\mid v} q$ in $\varphi'$.
		Any atom $\final(q)$ is replaced by $\final(f_Q(q)^\first)$ if there exists a binding $\exists \pi \colon q\xrightarrow{u\mid v} q'$ in $\varphi'$ otherwise $\final(q)$ is replaced by $\final(f_Q(q)^\last)$ and there exists a binding $\exists \pi \colon q'\xrightarrow{u\mid v} q$ in $\varphi'$.
	\item
		Finally, any atom $\pi=\pi'$ is replaced by $\pi=_\P \pi'$.
	\end{itemize}
	
	Now, $\varphi$ and $\psi$ are equivalent in the
	following sense. Any valuation $\nu$ satisfying
	$\varphi$ satisfies $\psi$ as well (if restricted to
	its path variables). Conversely for all valuations $\nu'$ satisfying
	$\psi$, we define the following valuation $\nu$:
	$$
		\begin{array}{lllllllll}
			\nu(\pi) & = & \nu'(\pi) &
				\text{for all path variables } \pi
		\smallskip\\
			\nu(u)  & = & \inp(\nu'(f_I(u))) &
				\text{for all input variables } u
		\smallskip\\
			\nu(v)  & = & \out(\nu'(f_O(v))) & \text{for all
				output variables }
			v
		\smallskip\\
			\nu(q) & = & (\nu'(f_Q(q)))^\first &
				\text{for all state variables $q$ such that there}\\
			& & &
				\text{exists a binding $\exists \pi:q\xrightarrow{u\mid v} q'$ in $\varphi$}
		\smallskip\\
			\nu(q) & = & (\nu'(f_Q(q)))^\last &
				\text{otherwise}
		\end{array}
	$$
	
	Then, $\nu$ satisfies $\varphi$. Hence, it is possible
	to recover all the models of $\varphi$ from the models
	of $\nu$.
	\qed
\end{proof}

The converse of the previous lemma, although not needed for the
purpose of this paper, holds as well. For all path formula one can
build in linear time a pattern formula which is satisfied over some
automaton $A$ iff the former is satisfied as well. 

% ----------------------------------------------------------------------- %


\begin{example}
	The pattern formula 
	$$
		\exists \pi_1\colon p\xrightarrow{u\mid v} q,
		\exists \pi_2 \colon p\xrightarrow{u'\mid v} q',
		p(v\oplus v) \land q\neq q'
	$$
	is first transformed into the pattern formula
	$$
		\exists \pi_1\colon p\xrightarrow{u\mid v} q,
		\exists \pi_2\colon p'\xrightarrow{u'\mid v'} q',
		p(v\oplus v)\land q\neq q'\land p=p'\land v = v'\land u\neq u'
	$$
	which in turn is transformed into the path formula 
	$$
		p(\pi_1\oplus \pi_1)\land
		\pi_1^\last\neq_Q \pi_2^\last\land
		\pi_1^\first=_Q \pi_2^\first\land
		\pi_1=_O \pi_2\land
		\pi_1\neq_I \pi_2
	$$
\end{example}


\subsection{Generic Model-Checking Algorithm}

First, the following lemma states that any predicate (or its negation) which
are not an output predicate, interpreted over runs of automata with
outputs, define a regular sets of run tuples. 

\begin{lemma}\label{lem:basic}
    Let $X = \{\pi_1,\dots,\pi_n\}$ be a finite set of (ordered) path
    variables and let $\{\pi'_1,\dots,\pi'_m\}\subseteq X$. Let $A$ be an automaton with outputs and $p(\pi'_1,\dots,\pi'_m)$ be
    some atomic path formula, where $p\in \{ \prefix_I, {\in_I} L, \leq_I^{len}, \init(.^d), \final(.^d),
    .^{d_1}=_Q.^{d_2}, =_P\}$ and $d,d_1,d_2\in \{\first,\last\}$.
    One can construct an NFA $M_{p}$ with a number of states
    exponential in $n$, such that 
    $$
    L(M_{p}) = \{ (\nu(\pi_1),\dots,\nu(\pi_n))\mid \nu:X\rightarrow
    \paths(A)\wedge \nu\in\sem{p(\pi'_1,\dots,\pi'_m)}_A\}
    $$
    One can construct an NFA $M_{\neg p}$ with a number of states
    exponential in $n$ (and exponential in the number of states of the
    NFA representing $L$ when $p$ is the predicate ${\in_I} L$), such that
    $$
    L(M_{\neg p}) = \{ (\nu(\pi_1),\dots,\nu(\pi_n))\mid \nu:X\rightarrow
    \paths(A)\wedge \nu\not\in\sem{p(\pi'_1,\dots,\pi'_m)}_A\}
    $$
\end{lemma}

\begin{proof}
    First , let $Q$ be the set of states of $A$ with initial states
    $Q_0$ and final states $Q_F$,  and let $D_f$ be the
    output values occurring on $A$. Let $\Sigma =
    \Lambda \cup Q \cup D_f \cup \{ \bot\}$. It is not difficult to
    construct an NFA $B$ over $\Sigma^n$ such that $L(B) =
    \paths(A)^n$. The NFA $B$ is the $n$-times product of $A$,
    augmented with intermediate states and transitions to read the
    states of $Q$ and the values in $D_f$ (seen as letters). This NFA
    has a number of states exponential in $n$ and an alphabet
    exponential in $n$ as well. 



    For a predicate $p(\pi'_1,\dots,\pi'_m)$ of the above type, we construct an NFA $B_p$
    (explained after) and $M_p$ is obtained as the product of $B$ and
    $B_p$, i.e. $M_p = B\otimes B_p$ and $L(M_p) = L(B)\cap L(B_p)$. 
    We now consider the different types $p$ can take case by
    case:
    
    \begin{itemize}
      \item Case $\pi_i\prefix_I \pi_j$: $B_p$ is given by the
        single-state automaton (with $|\Sigma|^n$ transitions)
			\begin{center}
				\drawPrefix
			\end{center}

                      \item Case $\pi_i \in L$. We construct an
                        automaton accepting the set of words
                        $w\in\Sigma^n$ such that $f(w)\in L$, where
                        $f$ is the morphism defined by
                        $f(\sigma_1,\dots,\sigma_n) = \epsilon$ if
                        $\sigma_i\not\in \Lambda$, and
                        $f(\sigma_1,\dots,\sigma_n) = \sigma_i$
                        otherwise, for all
                        $(\sigma_1,\dots,\sigma_n)\in\Sigma^n$. In
                        otherwords, $B_p$ recognises the language 
                        $f^{-1}(L)$. Since regular languages are
                        closed under inverse morphism, we get the
                        existence of $B_p$. We can construct from any NFA
                        $B_L$ recognising $L$ by replacing any 
                        transition $(q,\lambda,q')$ of $B_L$ by the
                        transitions $(q,\overline{\sigma},q')$ for all
                        $\overline{\sigma}\in\Sigma^n$ such that
                        $\overline{\sigma}_i = \lambda$, and by adding
                        intermediate states and transitions to $B_L$
                        reading letters whose $i$th component is not
                        in $\Lambda$. The resulting automaton is
                        exponential in $n$. 

		\item Case $\pi_i \leq^\text{len}_I \pi_j$. By the
                  definition of convolution, it suffices to check that
                  whenever the $j$th component of a letter
                  $\overline{\sigma}\in\Sigma^n$ is $\bot$, then so is
                  its $i$th component. This is done by the
                  single-state automaton
			\begin{center}
				\drawSize
			\end{center}
		\item Case $\pi_i =_P \pi_j$. It suffices to check that
                  the $i$th and $j$th components are the same:
			\begin{center}
				\drawPathEqual
			\end{center}
		\item Cases $\init(\pi_i^\vartriangleleft)$ and $\final(\pi_i^\vartriangleleft)$. The automata
                  $B_p$ are respectively:
                  \begin{center}
                  \drawStateLeftInit
                  \smallskip\\
                  \drawStateLeftFinal
              \end{center}                  

		\item Cases $\init(\pi_i^\vartriangleright)$ and $\final(\pi_i^\vartriangleright)$. The automata
                  $B_p$ are respectively:
                  \begin{center}
                  \drawStateRightInit
                  \smallskip\\
                  \drawStateRightFinal
              \end{center}                  

		\item Case $\pi_i^{d_1} = \pi_j^{d_2}$
                  with $d_1, d_2 \in \{ \vartriangleleft,
                  \vartriangleright \}$. The constructions are similar
                  as before. For instance, take the constraint
                  $\pi_i^\vartriangleleft =
                  \pi_j^\vartriangleright$. Then, the automaton $B_p$
                  needs to remember (in its control state) the first state of $A$ read on the $i$th
                  component and checks later on that it is equal to
                  the last state read on the $j$th component. Since
                  again result in automata exponential in $n$. 

		% \item
			% Case $\varphi \equiv \lnot \varphi_1$.
			% By induction hypothesis applied on $\varphi_1$, we can construct $B_1$ such that $\sem{\varphi_1}_A = \paths(A)^{n} \cap L(B_1)$.
			% $$
				% \begin{array}{ll}
					% \sem{\varphi}_A &= \paths(A)^{n} \setminus \sem{\varphi_1}_A
				% \\
					% &=\paths(A)^{n} \cap \left( \paths(A)^{n} \cap L_1^\sharp \right)^c
				% \\
					% &= \paths(A)^{n} \cap \left(L(B_1)^c\right)^\sharp
				% \end{array}
			% $$
		% \item
			% Case $\varphi \equiv \varphi_1 \land \varphi_2$.
			% For $1 \leq i \leq 2$, by induction hypothesis applied on $\varphi_i$, we can construct $B_i$ such that $\sem{\varphi_i}_A = \paths(A)^{n} \cap L(B_i)$.
			% $$
				% \begin{array}{ll}
					% \sem{\varphi}_A &= \sem{\varphi_1}_A \cap \sem{\varphi_2}_A
				% \\
					% &= \left( \paths(A)^{n} \cap L(B_1)^\sharp \right) \cap \left( \paths(A)^{n} \cap L(B_2)^\sharp \right)
				% \\
					% &= \paths(A)^{n} \cap \left( L(B_1) \cap L(B_2) \right)^\sharp
				% \end{array}
			% $$
		% \item
			% Case $\varphi \equiv \varphi_1 \lor \varphi_2$.
			% For $1 \leq i \leq 2$, by induction hypothesis applied on $\varphi_i$, we can construct $L_i$ such that $\sem{\varphi_i}_A = \paths(A)^{n} \cap L(B_i)$.
			% $$
				% \begin{array}{ll}
					% \sem{\varphi}_A &= \sem{\varphi_1}_A \cup \sem{\varphi_2}_A
				% \\
					% &= \left( \paths(A)^{n} \cap L(B_1)^\sharp \right) \cup \left( \paths(A)^{n} \cap L(B_2)^\sharp \right)
				% \\
					% &= \paths(A)^{n} \cap \left( L(B_1) \cup L(B_2) \right)^\sharp
				% \end{array}
			% $$
		\end{itemize}

                For the case of negation, we construct the complement
                of the automata $B_p$ constructed before. For all
                cases but the predicate ${\in_I} L$, they have a
                constant number of states and therefore can be
                complemented in polynomial time (hence in exponential
                time in $n$). For the predicate $\neg (\pi_i {\in_I}
                L)$, we first rewrite it into $\pi_i\in_I
                \overline{L}$, which causes an exponential in the
                number of states of the NFA recognising $L$. \qed
\end{proof}

\begin{algorithm}\caption{Generic Model-Checking Algorithm}\label{algoG}
	\DontPrintSemicolon
	\SetKwInput{In}{Inputs}
	\SetKwInput{Out}{Output}
	\SetKwInput{Assumption}{Assumption}
	\SetKwFunction{acceptor}{buildAcceptor}
	\SetKwFunction{match}{patternMatching}
	\SetKwProg{funacceptor}{Function}{$\colon \C|_n$}{end}
	\SetKwProg{funmatch}{Function}{$\colon \bool$}{}
	\SetKw{with}{with}
	\SetKw{bool}{boolean}
	
	\In{\text{}
		\\\quad\ A pattern formula $\psi$ over a set of output
                predicates $\O$
		\\\quad\ An automaton $A$ with output over a monoid
                $\M = (D,\oplus_\M,\zero_\M)$
	}
	\Out{Decide $A \models \psi$}
	\Assumption{\text{} There exists a class of path acceptors
          $\C$ effectively good for $\M$ and $\O$.
	}
	\BlankLine
	
	\funacceptor{\acceptor{$\varphi \colon \logic_P(\O),X=(\pi_1,\dots,\pi_n)$}}{
          \tcc*[l]{$\varphi$ is assumed to be in negation normal form}
		\ShowLn
		\uIf{$\varphi \equiv p(\pi'_{1},\dots,\pi'_{k})$
                  \with $p\in\O$}{
			\Return{$M_{p}$ such that $\sem{M_p} = \{
                          (\nu(\pi_1),\dots,\nu(\pi_n))\mid
                          \nu:X\rightarrow \paths(A)\wedge \nu\in\sem{l(\pi'_1,\dots,\pi'_j)}_A\}$}\;
			\tcc*[l]{exists by condition \ref{goodout} of
                          a good class}
		}
		\ShowLn
		\uIf{$\varphi \equiv \neg p(\pi'_{1},\dots,\pi'_{k})$
                  \with $p\in\O$}{
                \tcc*[l]{this case can only happen if $\varphi\not\in\logic_P^+(\O)$}
			\Return{$M_{\neg p}$ such that $\sem{M_{\neg p}} = \{
                          (\nu(\pi_1),\dots,\nu(\pi_n))\mid
                          \nu:X\rightarrow \paths(A)\wedge \nu\not\in\sem{l(\pi'_1,\dots,\pi'_j)}_A\}$}\;
			\tcc*[l]{exists by condition \ref{goodout-neg} of
                          a good class}
		}
		\ShowLn
		\uIf{$\varphi \equiv l$ \with $l = p$ or $l=\neg p$
                  where $p\not\in \O$}{
			\Return{$M_{l}$ such that $\sem{M_l} = \{
                          (\nu(\pi_1),\dots,\nu(\pi_n))\mid
                          \nu:X\rightarrow \paths(A)\wedge \nu\in\sem{l(\pi'_1,\dots,\pi'_j)}_A\}$}\;
			\tcc*[l]{exists by Lemma~\ref{lem:basic} and condition \ref{goodreg} of good class}
		}
		\ShowLn
		\uIf{$\varphi \equiv \varphi_1 \lor \varphi_2$ }{
			$M_1 \affect \acceptor{$\varphi_1$}$\;
			$M_2 \affect \acceptor{$\varphi_2$}$\;
			\Return{$M_1 \cup M_2$}\;
			\tcc*[l]{exists by condition \ref{goodclos} of good class}
		}
		\ShowLn
		\If{$\varphi \equiv \varphi_1 \land \varphi_2$}{
			$M_1 \affect \acceptor{$\varphi_1$}$\;
			$M_2 \affect \acceptor{$\varphi_2$}$\;
			\Return{$M_1 \cap M_2$}\;
			\tcc*[l]{exists by condition \ref{goodclos} of good class}
		}
	}
	\BlankLine
	
	\funmatch{\match{$A,\psi$}}{
		\ShowLn
                $\phi\affect$ path formula equivalent to $\psi$\;
                \tcc*[r]{Exists by Lemma~\ref{lem:translate}}
		\ShowLn
                $\varphi\affect $ negation normal form of $\varphi$\;
		\ShowLn
                $\{\pi_1,\dots,\pi_n\}\affect$ path variables of
                $\varphi$ (arbitrarily ordered)\;
		\ShowLn
		$M \affect$ \acceptor{$A,\phi,\{\pi_1,\dots,\pi_n\}$}\;
		\ShowLn
		\Return{$\sem{M} \neq \varnothing$}\;
		\tcc*[l]{Is decidable by effectiveness of $\C$}
		%\tcc*[l]{since $\C$ is an effective good class}
	}
\end{algorithm}




% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "app-mc.tex"
%%% End:


==> app-mc.tex <==
\section{Model-Checking Problem -- Section~\ref{sec:MC}}

\subsection{An intermediate syntax for formulas}

In the pattern logic, we have four types of variables (paths, states, inputs and outputs).
While this is appealing for succinctness and readability reasons, it is less easy to deal with at an algorithmic level.
Therefore, we introduce here another syntax, called path formulas, in which there is a single type of variables: path variables.
We then show that the two logics are equivalent in the sense that satisfiability by any automaton with output is preserved. 


% ----------------------------------------------------------------------- %


\begin{definition}
	Let $X$ a set of path variables and $\O$ a set of output predicates.
	A \emph{path formula} $\varphi$ over $\O$ is a term generated by the following grammar:
	$$
		\begin{array}{lcll}
			\text{path formula} & \varphi \Coloneqq &
				\varphi \land \varphi \mid
				\varphi \lor \varphi \mid
				\lnot \varphi \mid
		\smallskip\\
			\text{input constraints} &&
				\pi_1 \prefix_I \pi_2 \mid
				\pi \in_I L \mid
				\pi_1 \leq^\text{len}_I \pi_2 \mid
		\smallskip\\
			\text{state constraints} &&
				\init(\pi^d) \mid
				\final(\pi^d) \mid
				\pi_1^{d_1} =_Q \pi_2^{d_2} \mid 
		\smallskip\\ 
			\text{path constraints} &&
				\pi_1 =_P \pi_2
		\smallskip\\
			\text{output constraints} &&
				p(t_1,\dots,t_{\alpha(p)})
				%& \forall p\in\O
		\end{array}
	$$
	where $\pi,\pi_1,\pi_2\in X$, $d,d_1,d_2\in\{\first,\last\}$
	$t_1,\dots,t_n\in \text{Terms}(X,\oplus,\zero)$,
	$p \in \O$ of arity $\alpha(p)$ and
	$L$ ranges over regular languages over $\Lambda$.
	We denote by $\logic_P(\O)$ the set of path formulas over
        $\O$, and by $\logic_P^+(\O)$ its fragment where output
        predicates does not occur under an odd number of negations. 
\end{definition}

We introduce usual syntactic sugar:
$(\pi =_I \pi') \new \pi\prefix_I \pi' \land  \pi'\prefix_I \pi$,
$(\pi=^\text{len}_I \pi') \new (\pi\leq^\text{len}_I \pi')\land (\pi'\leq^\text{len}_I \pi)$,
$(\pi<^\text{len}_I \pi') \new \lnot (\pi'\leq^\text{len}_I \pi)$,

Informally, path formulas only speak about the paths of an automaton
with output, the input constraints speak about properties of their
inputs, the state contraints about properties of their starting and
ending states, and $\O$ about properties of their outputs.
The semantics of such a formula is then, on an automaton with output
$A$, valuations of path variables into paths in $\paths(A)$. 


Formally, we first fix some monoid $\M = (D,\oplus_\M,\zero_\M)$ together with an interpretation ${p}^\M$ of each output predicate $p \in \O$.
Let $A \in \trs(\M)$ be an automaton with output. Given a valuation
$\nu\colon X\rightarrow \paths(A)$, the interpretation $t^{\nu,\M}\in
D$ of terms $t\in\text{Terms}(X,\oplus,\zero)$ is inductively defined
by $(t_1\oplus t_2)^{\nu,\M} = t_1^{\nu,\M}\oplus t_2^{\nu,\M}$,
$\zero^{\nu,\M} = \zero_\M$ and $\pi^{\nu,\M} = \out(\nu(\pi))\in D$. Then a formula $\varphi \in
\logic_P(\O)$ is interpreted in $A= (Q, I, F, \Delta, \gamma)$ as a
set of valuations denoted $\sem{\varphi}_A\subseteq\paths(A)^{X}$ defined as follows.
$$
	\begin{array}{l}
		\sem{\init(\pi^d)}_A = \{ \nu \  \mid \nu(\pi)^d \in I \}
	\smallskip\\
		\sem{\pi_1^{d_1} =_Q \pi_2^{d_2}}_A = \{ \nu \  \mid \nu(\pi_1)^{d_1} = \nu(\pi_2)^{d_2} \}
	\smallskip\\
		\sem{\final(\pi^d)}_A = \{ \nu \  \mid \nu(\pi)^d \in F \}
	\smallskip\\
		\sem{\lnot\varphi}_A = \paths(A)^{X} \setminus \sem{\varphi}_A
	\smallskip\\
		\sem{\varphi_1 \land \varphi_2}_A = \sem{\varphi_1}_A \cap \sem{\varphi_2}_A
	\smallskip\\
		\sem{\varphi_1 \lor \varphi_2}_A = \sem{\varphi_1}_A \cup \sem{\varphi_2}_A
	\smallskip\\
		\sem{\pi_1 \prefix_I \pi_2}_A = \{ \nu \  \mid \inp(\nu(\pi_1)) \prefix \inp(\nu(\pi_2)) \}
	\smallskip\\
		\sem{\pi_1 =_P \pi_2}_A = \{ \nu \  \mid \nu(\pi_1) = \nu(\pi_2) \}
	\smallskip\\
		\sem{\pi_1 \leq^{len}_I \pi_2}_A = \{ \nu \  \mid |\inp(\nu(\pi_1))| \leq |\inp(\nu(\pi_2))| \}
	\smallskip\\
		\sem{\pi \in_I L}_A = \{ \nu \  \mid \inp(\nu(\pi)) \in L \}
	\smallskip\\
		\sem{p(t_1,\dots,t_{\alpha(p)})}_A = \{ \nu \  \mid (t_1^{\nu, \M},\dots,t_{\alpha(p)}^{\nu, \M}) \in p^\M\}
	\end{array}
$$
A path formula $\varphi$ is said to be satisfiable over $A$ if
$\sem{\varphi}_A \neq \varnothing$. The path logic and the pattern
logic are equivalent in the following precise sense. 


% ----------------------------------------------------------------------- %


\begin{lemma} \label{lem:translate}
	For all pattern formulas $\varphi \in \logic(\O)$, 
        (resp. $\varphi\in\logic^+(\O)$), one can construct in linear
        time a path formula $\psi \in \logic_P(\O\cup\{=_O\})$
        (resp. $\psi\in\logic_P^+(\O\cup \{=_O\})$) such
        that the following hold:
	\begin{enumerate}
	\item
		$\Var_P(\varphi) = \Var(\psi)$
	\item
		for all monoid $\M = (D,\oplus_\M,\zero_\M)$,
		all interpretation $p^\M \in D^{\alpha(p)}$ for each $p \in \O$,
		all automata with output $A \in \trs(\M)$,  we have $A\models \varphi$ iff $A\models \psi$
		\item there is a surjective mapping from the valuations (in $A$)  satisfying $\psi$ to the valuations satisfying $\varphi$. 
	\end{enumerate}
	In addition, if $\varphi$ does not contain twice the same output variable in its prefix, then $\psi \in \logic_P(\O)$.
\end{lemma}

\begin{proof}
	Assume that $\varphi$ is of the form:
	$$
	\exists \pi_1:p_1\xrightarrow{u_1\mid
		v_1} q_1\ldots \exists \pi_n:p_n\xrightarrow{u_n\mid
		v_n} q_n\cdot \mathcal{C}
	$$
	In a first step, we rename the $j$-th occurrences, $j>1$, of any
	state, input and output variables so that eventually, all these
	variables are pairwise different in the prefix. This can be easily
	done in linear-time modulo adding some equality constraints to
	$\mathcal{C}$. For instance, if we have $p_i = p_j$, $i<j$, we use
	a fresh variable name $p$ and replace $p_j$ by $p$ in the prefix
	$\exists \pi_1\dots \exists \pi_n$, and add the constraint $p =
	p_i$ to $\mathcal{C}$. We do the same for the other types of
	variables. Note that it is not necessary to do it for the path
	variables $\pi_i$, since by definition of pattern formulas, they
	are assumed to occur only once in the prefix. 
	
	
	We end up with a formula of the form 
	$$
	\varphi' \equiv \exists \pi_1:p'_1\xrightarrow{u'_1\mid
		v'_1} q'_1\ldots \exists \pi_n:p'_n\xrightarrow{u'_n\mid
		v'_n} q'_n\cdot \mathcal{C'}
	$$
	where all the variables occur once in the prefix,
	together with a mapping $f$ from the new variables to
	the old ones. We also assume that $f$ is the identify
	on the path variables. In our previous example, we would have
	$f(p) = p_j$ for instance. 
	
	Then, $\varphi'$ and $\varphi$ are equivalent in the
	following sense: over an automaton with output, for all 
	valuations $\nu$ satisfying $\varphi$, $\nu\circ
	f$ satisfies $\varphi'$. Conversely, for all
	valuations $\nu'$ satisfying $\varphi'$, the valuation 
	$\nu'$ restricted to the variables of $\varphi$
	satisfies $\varphi$. Hence, it is possible to recover
	the models of $\varphi$ from the models of $\varphi'$,
	and conversely. 
	
	Now, note that in $\varphi'$, there is a functional
	dependency between the state, input and output
	variables, and the path variables. This dependency is
	formalised through three functions $f_Q, f_I, f_O$
	from respectively,
	$\{p'_1,\dots,p'_n,q'_1,\dots,q'_n\}$ to
	$\{\pi_1,\dots,\pi_n\}$, $\{ u'_1,\dots,u'_n\}$ to 
	$\{\pi_1,\dots,\pi_n\}$, and from $\{
	v'_1,\dots,v'_n\}$ to $\{\pi_1,\dots,\pi_n\}$. 
	
	Then, $\psi$ is obtained by applying the following
	transformations on $\mathcal{C}$:
	\begin{itemize}
	\item
		Any atom $u\prefix u'$ is replaced by $f_I(u)\prefix_I f_I(u')$.
		Any atom $u\in L$ by $f_I(u)\in_I L$.
		Any atom $|u|\leq |u'|$ by $f_I(u) \leq_I^\text{len} f_I(u')$.
	\item
		Any atom $p(t_1,\dots,t_k)$ is replaced by $p(t'_1,\dots,t'_k)$ where $t'_i$ is obtained by substituting any variable $v$ in $t_i$ by $f_O(v)$.
	\item
		Any atom $\init(q)$ is replaced by $\init(f_Q(q)^\first)$ if there exists a binding $\exists \pi \colon q\xrightarrow{u\mid v} q'$ in $\varphi'$ otherwise $\init(q)$ is replaced by $\init(f_Q(q)^\last)$ and there exists a binding $\exists \pi \colon q'\xrightarrow{u\mid v} q$ in $\varphi'$.
		Any atom $\final(q)$ is replaced by $\final(f_Q(q)^\first)$ if there exists a binding $\exists \pi \colon q\xrightarrow{u\mid v} q'$ in $\varphi'$ otherwise $\final(q)$ is replaced by $\final(f_Q(q)^\last)$ and there exists a binding $\exists \pi \colon q'\xrightarrow{u\mid v} q$ in $\varphi'$.
	\item
		Finally, any atom $\pi=\pi'$ is replaced by $\pi=_\P \pi'$.
	\end{itemize}
	
	Now, $\varphi$ and $\psi$ are equivalent in the
	following sense. Any valuation $\nu$ satisfying
	$\varphi$ satisfies $\psi$ as well (if restricted to
	its path variables). Conversely for all valuations $\nu'$ satisfying
	$\psi$, we define the following valuation $\nu$:
	$$
		\begin{array}{lllllllll}
			\nu(\pi) & = & \nu'(\pi) &
				\text{for all path variables } \pi
		\smallskip\\
			\nu(u)  & = & \inp(\nu'(f_I(u))) &
				\text{for all input variables } u
		\smallskip\\
			\nu(v)  & = & \out(\nu'(f_O(v))) & \text{for all
				output variables }
			v
		\smallskip\\
			\nu(q) & = & (\nu'(f_Q(q)))^\first &
				\text{for all state variables $q$ such that there}\\
			& & &
				\text{exists a binding $\exists \pi:q\xrightarrow{u\mid v} q'$ in $\varphi$}
		\smallskip\\
			\nu(q) & = & (\nu'(f_Q(q)))^\last &
				\text{otherwise}
		\end{array}
	$$
	
	Then, $\nu$ satisfies $\varphi$. Hence, it is possible
	to recover all the models of $\varphi$ from the models
	of $\nu$.
	\qed
\end{proof}

The converse of the previous lemma, although not needed for the
purpose of this paper, holds as well. For all path formula one can
build in linear time a pattern formula which is satisfied over some
automaton $A$ iff the former is satisfied as well. 

% ----------------------------------------------------------------------- %


\begin{example}
	The pattern formula 
	$$
		\exists \pi_1\colon p\xrightarrow{u\mid v} q,
		\exists \pi_2 \colon p\xrightarrow{u'\mid v} q',
		p(v\oplus v) \land q\neq q'
	$$
	is first transformed into the pattern formula
	$$
		\exists \pi_1\colon p\xrightarrow{u\mid v} q,
		\exists \pi_2\colon p'\xrightarrow{u'\mid v'} q',
		p(v\oplus v)\land q\neq q'\land p=p'\land v = v'\land u\neq u'
	$$
	which in turn is transformed into the path formula 
	$$
		p(\pi_1\oplus \pi_1)\land
		\pi_1^\last\neq_Q \pi_2^\last\land
		\pi_1^\first=_Q \pi_2^\first\land
		\pi_1=_O \pi_2\land
		\pi_1\neq_I \pi_2
	$$
\end{example}


\subsection{Model-Checking Algorithm}

% ----------------------------------------------------------------------- %
First, the following lemma states that any predicate (or its negation) which
are not an output predicate, interpreted over paths of automata with
outputs, define a regular sets of path tuples. 

\begin{lemma}\label{lem:basic}
    Let $X = \{\pi_1,\dots,\pi_n\}$ be a finite set of (ordered) path
    variables and let $\{\pi'_1,\dots,\pi'_m\}\subseteq X$. Let $A$ be an automaton with outputs and $p(\pi'_1,\dots,\pi'_m)$ be
    some atomic path formula, where $p\in \{ \prefix_I, {\in_I} L, \leq_I^{len}, \init(.^d), \final(.^d),
    .^{d_1}=_Q.^{d_2}, =_P\}$ and $d,d_1,d_2\in \{\first,\last\}$.
    One can construct an NFA $M_{p}$ with a number of states
    exponential in $n$, such that 
    $$
    L(M_{p}) = \{ (\nu(\pi_1),\dots,\nu(\pi_n))\mid \nu:X\rightarrow
    \paths(A)\wedge \nu\in\sem{p(\pi'_1,\dots,\pi'_m)}_A\}
    $$
    One can construct an NFA $M_{\neg p}$ with a number of states
    exponential in $n$ (and exponential in the number of states of the
    NFA representing $L$ when $p$ is the predicate ${\in_I} L$), such that
    $$
    L(M_{\neg p}) = \{ (\nu(\pi_1),\dots,\nu(\pi_n))\mid \nu:X\rightarrow
    \paths(A)\wedge \nu\not\in\sem{p(\pi'_1,\dots,\pi'_m)}_A\}
    $$
\end{lemma}

\begin{proof}
    First , let $Q$ be the set of states of $A$ with initial states
    $Q_0$ and final states $Q_F$,  and let $D_f$ be the
    output values occurring on $A$. Let $\Sigma =
    \Lambda \cup Q \cup D_f \cup \{ \bot\}$. It is not difficult to
    construct an NFA $B$ over $\Sigma^n$ such that $L(B) =
    \paths(A)^n$. The NFA $B$ is the $n$-times product of $A$,
    augmented with intermediate states and transitions to read the
    states of $Q$ and the values in $D_f$ (seen as letters). This NFA
    has a number of states exponential in $n$ and an alphabet
    exponential in $n$ as well. 



    For a predicate $p(\pi'_1,\dots,\pi'_m)$ of the above type, we construct an NFA $B_p$
    (explained after) and $M_p$ is obtained as the product of $B$ and
    $B_p$, i.e. $M_p = B\otimes B_p$ and $L(M_p) = L(B)\cap L(B_p)$. 
    We now consider the different types $p$ can take case by
    case:
    
    \begin{itemize}
      \item Case $\pi_i\prefix_I \pi_j$: $B_p$ is given by the
        single-state automaton (with $|\Sigma|^n$ transitions)
			\begin{center}
				\drawPrefix
			\end{center}

                      \item Case $\pi_i \in L$. We construct an
                        automaton accepting the set of words
                        $w\in\Sigma^n$ such that $f(w)\in L$, where
                        $f$ is the morphism defined by
                        $f(\sigma_1,\dots,\sigma_n) = \epsilon$ if
                        $\sigma_i\not\in \Lambda$, and
                        $f(\sigma_1,\dots,\sigma_n) = \sigma_i$
                        otherwise, for all
                        $(\sigma_1,\dots,\sigma_n)\in\Sigma^n$. In
                        otherwords, $B_p$ recognises the language 
                        $f^{-1}(L)$. Since regular languages are
                        closed under inverse morphism, we get the
                        existence of $B_p$. We can construct from any NFA
                        $B_L$ recognising $L$ by replacing any 
                        transition $(q,\lambda,q')$ of $B_L$ by the
                        transitions $(q,\overline{\sigma},q')$ for all
                        $\overline{\sigma}\in\Sigma^n$ such that
                        $\overline{\sigma}_i = \lambda$, and by adding
                        intermediate states and transitions to $B_L$
                        reading letters whose $i$th component is not
                        in $\Lambda$. The resulting automaton is
                        exponential in $n$. 

		\item Case $\pi_i \leq^\text{len}_I \pi_j$. By the
                  definition of convolution, it suffices to check that
                  whenever the $j$th component of a letter
                  $\overline{\sigma}\in\Sigma^n$ is $\bot$, then so is
                  its $i$th component. This is done by the
                  single-state automaton
			\begin{center}
				\drawSize
			\end{center}
		\item Case $\pi_i =_P \pi_j$. It suffices to check that
                  the $i$th and $j$th components are the same:
			\begin{center}
				\drawPathEqual
			\end{center}
		\item Cases $\init(\pi_i^\vartriangleleft)$ and $\final(\pi_i^\vartriangleleft)$. The automata
                  $B_p$ are respectively:
                  \begin{center}
                  \drawStateLeftInit
                  \smallskip\\
                  \drawStateLeftFinal
              \end{center}                  

		\item Cases $\init(\pi_i^\vartriangleright)$ and $\final(\pi_i^\vartriangleright)$. The automata
                  $B_p$ are respectively:
                  \begin{center}
                  \drawStateRightInit
                  \smallskip\\
                  \drawStateRightFinal
              \end{center}                  

		\item Case $\pi_i^{d_1} = \pi_j^{d_2}$
                  with $d_1, d_2 \in \{ \vartriangleleft,
                  \vartriangleright \}$. The constructions are similar
                  as before. For instance, take the constraint
                  $\pi_i^\vartriangleleft =
                  \pi_j^\vartriangleright$. Then, the automaton $B_p$
                  needs to remember (in its control state) the first state of $A$ read on the $i$th
                  component and checks later on that it is equal to
                  the last state read on the $j$th component. Since
                  again result in automata exponential in $n$. 

		% \item
			% Case $\varphi \equiv \lnot \varphi_1$.
			% By induction hypothesis applied on $\varphi_1$, we can construct $B_1$ such that $\sem{\varphi_1}_A = \paths(A)^{n} \cap L(B_1)$.
			% $$
				% \begin{array}{ll}
					% \sem{\varphi}_A &= \paths(A)^{n} \setminus \sem{\varphi_1}_A
				% \\
					% &=\paths(A)^{n} \cap \left( \paths(A)^{n} \cap L_1^\sharp \right)^c
				% \\
					% &= \paths(A)^{n} \cap \left(L(B_1)^c\right)^\sharp
				% \end{array}
			% $$
		% \item
			% Case $\varphi \equiv \varphi_1 \land \varphi_2$.
			% For $1 \leq i \leq 2$, by induction hypothesis applied on $\varphi_i$, we can construct $B_i$ such that $\sem{\varphi_i}_A = \paths(A)^{n} \cap L(B_i)$.
			% $$
				% \begin{array}{ll}
					% \sem{\varphi}_A &= \sem{\varphi_1}_A \cap \sem{\varphi_2}_A
				% \\
					% &= \left( \paths(A)^{n} \cap L(B_1)^\sharp \right) \cap \left( \paths(A)^{n} \cap L(B_2)^\sharp \right)
				% \\
					% &= \paths(A)^{n} \cap \left( L(B_1) \cap L(B_2) \right)^\sharp
				% \end{array}
			% $$
		% \item
			% Case $\varphi \equiv \varphi_1 \lor \varphi_2$.
			% For $1 \leq i \leq 2$, by induction hypothesis applied on $\varphi_i$, we can construct $L_i$ such that $\sem{\varphi_i}_A = \paths(A)^{n} \cap L(B_i)$.
			% $$
				% \begin{array}{ll}
					% \sem{\varphi}_A &= \sem{\varphi_1}_A \cup \sem{\varphi_2}_A
				% \\
					% &= \left( \paths(A)^{n} \cap L(B_1)^\sharp \right) \cup \left( \paths(A)^{n} \cap L(B_2)^\sharp \right)
				% \\
					% &= \paths(A)^{n} \cap \left( L(B_1) \cup L(B_2) \right)^\sharp
				% \end{array}
			% $$
		\end{itemize}

                For the case of negation, we construct the complement
                of the automata $B_p$ constructed before. For all
                cases but the predicate ${\in_I} L$, they have a
                constant number of states and therefore can be
                complemented in polynomial time (hence in exponential
                time in $n$). For the predicate $\neg (\pi_i {\in_I}
                L)$, we first rewrite it into $\pi_i\in_I
                \overline{L}$, which causes an exponential in the
                number of states of the NFA recognising $L$. \qed
\end{proof}

\begin{algorithm}\caption{Generic Model-Checking Algorithm}\label{algoG}
	\DontPrintSemicolon
	\SetKwInput{In}{Inputs}
	\SetKwInput{Out}{Output}
	\SetKwInput{Assumption}{Assumption}
	\SetKwFunction{acceptor}{buildAcceptor}
	\SetKwFunction{match}{patternMatching}
	\SetKwProg{funacceptor}{Function}{$\colon \C|_n$}{end}
	\SetKwProg{funmatch}{Function}{$\colon \bool$}{}
	\SetKw{with}{with}
	\SetKw{bool}{boolean}
	
	\In{\text{}
		\\\quad\ A pattern formula $\psi$ over a set of output
                predicates $\O$
		\\\quad\ An automaton $A$ with output over a monoid
                $\M = (D,\oplus_\M,\zero_\M)$
	}
	\Out{Decide $A \models \psi$}
	\Assumption{\text{} There exists a class of tuple-acceptors
          $\C$ effectively good for $\M$ and $\O$.
	}
	\BlankLine
	
	\funacceptor{\acceptor{$\varphi \colon \logic_P(\O),X=(\pi_1,\dots,\pi_n)$}}{
          \tcc*[l]{$\varphi$ is assumed to be a path formula in negation normal form}
		\ShowLn
		\uIf{$\varphi \equiv p(\pi'_{1},\dots,\pi'_{k})$
                  \with $p\in\O$}{
			\Return{$M_{p}$ such that $\sem{M_p} = \{
                          (\nu(\pi_1),\dots,\nu(\pi_n))\mid
                          \nu:X\rightarrow \paths(A)\wedge \nu\in\sem{l(\pi'_1,\dots,\pi'_j)}_A\}$}\;
			\tcc*[l]{exists by condition \ref{goodout} of
                          a good class}
		}
		\ShowLn
		\uIf{$\varphi \equiv \neg p(\pi'_{1},\dots,\pi'_{k})$
                  \with $p\in\O$}{
                \tcc*[l]{this case can only happen if $\varphi\not\in\logic_P^+(\O)$}
			\Return{$M_{\neg p}$ such that $\sem{M_{\neg p}} = \{
                          (\nu(\pi_1),\dots,\nu(\pi_n))\mid
                          \nu:X\rightarrow \paths(A)\wedge \nu\not\in\sem{l(\pi'_1,\dots,\pi'_j)}_A\}$}\;
			\tcc*[l]{exists by condition \ref{goodneg} of
                          a good class}
		}
		\ShowLn
		\uIf{$\varphi \equiv l$ \with $l = p$ or $l=\neg p$
                  where $p\not\in \O$}{
			\Return{$M_{l}$ such that $\sem{M_l} = \{
                          (\nu(\pi_1),\dots,\nu(\pi_n))\mid
                          \nu:X\rightarrow \paths(A)\wedge \nu\in\sem{l(\pi'_1,\dots,\pi'_j)}_A\}$}\;
			\tcc*[l]{exists by Lemma~\ref{lem:basic} and condition \ref{goodreg} of good class}
		}
		\ShowLn
		\uIf{$\varphi \equiv \varphi_1 \lor \varphi_2$ }{
			$M_1 \affect \acceptor{$\varphi_1$}$\;
			$M_2 \affect \acceptor{$\varphi_2$}$\;
			\Return{$M_1 \cup M_2$}\;
			\tcc*[l]{exists by condition \ref{goodclos} of good class}
		}
		\ShowLn
		\If{$\varphi \equiv \varphi_1 \land \varphi_2$}{
			$M_1 \affect \acceptor{$\varphi_1$}$\;
			$M_2 \affect \acceptor{$\varphi_2$}$\;
			\Return{$M_1 \cap M_2$}\;
			\tcc*[l]{exists by condition \ref{goodclos} of good class}
		}
	}
	\BlankLine
	
	\funmatch{\match{$A,\psi$}}{
		\ShowLn
                $\phi\affect$ path formula equivalent to $\psi$
                \tcc*[r]{Exists by Lemma~\ref{lem:translate}}
                \;
		\ShowLn
                $\varphi\affect $ negation normal form of $\varphi$\;
		\ShowLn
                $\{\pi_1,\dots,\pi_n\}\affect$ path variables of
                $\varphi$ (arbitrarily ordered)\;
		\ShowLn
		$M \affect$ \acceptor{$A,\phi,\{\pi_1,\dots,\pi_n\}$}\;
		\ShowLn
		\Return{$\sem{M} \neq \varnothing$}
		\tcc*[r]{Is decidable by effectiveness of $\C$}
		\;
	}
\end{algorithm}


This lemma can be generalised to any path formula as long as a an
effectively good class of path tuple acceptors exists: 

\begin{lemma}\label{lem:buildacceptor}
    Let $\C$ be an effectively good class (effectively weakly good
    class) of path tuple acceptors for
    an output monoid $\M$ and a set of output predicates $\O$. Let $A$
    be an automaton with outputs in $\M$ and let
    $\varphi\in\logic_P(\O)$ (resp. $\varphi\in\logic_P^+(\O)$) be a path formula with $X =
    \{\pi_1,\dots,\pi_n\}$ the variables occurring in $\varphi$. 
    One can construct a path tuple acceptor $M\in \C|_n$ such that 
    $$
    \sem{M} = \{ (\nu(\pi_1),\dots,\nu(\pi_n))\mid \nu:X\rightarrow
      \paths(A)\wedge \nu\in\sem{\varphi}_A\}
    $$
\end{lemma}



\subsubsection{Proof of Lemma~\ref{lem:buildacceptor}}

\begin{proof}
    The proof is given by the function $\acceptor$ of
    Algorithm~\ref{algoG}, which is assumed to run on a path formula
    in negation normal form (any path formula can be transformed into
    such a formula in linear time). \qed
\end{proof}


\subsection{Proof of Theorem~\ref{thm:algo}}

\begin{proof}
    First, by Lemma~\ref{lem:translate} we can effectively transform (in
    polynomial time) the input pattern formula $\psi$ into an
    equivalent path formula $\varphi$, which can be put in negation
    normal form (in linear-time). Let $X = \{\pi_1,\dots,\pi_n\}$ be
    the variables of $\varphi$. By Lemma~\ref{lem:buildacceptor}, one can
    effectively construct from $A, X$ and $\varphi$ a tuple
    acceptor $M\in\C|_n$ such that 
    $$
    \sem{M} = \{ (\nu(\pi_1),\dots,\nu(\pi_n))\mid \nu:X\rightarrow
    \paths(A)\wedge \nu\in\sem{\varphi}_A\}
    $$
    By the equivalence between $\varphi$ and $\psi$
    (Lemma~\ref{lem:translate}), we have $\sem{M}\neq \varnothing$ iff
    $A\models \psi$, which is decidable since $\C$ is effectively
    good. \qed
\end{proof}


% % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % % %



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "app-logic.tex"
%%% End:


==> app-nfa.tex <==
\section{A pattern logic for finite automata -- Section
  \ref{sec:regular}}


\subsection{Proof of Theorem~\ref{thm:mainNFA}}



\begin{proof}
	We start by showing the upper bounds.
	Let set $\psi \in \logic_\nfa$ a pattern formula and $A$ some NFA.
	This proof, presents an algorithm which decides $\varphi \models
        A$ in \textsc{NPSpace} and is in \textsc{NLogSpace} when
        the formula is fixed.


	First, note that NFAs are obviously an effectively good class of tuple-acceptors for the trivial monoid and $\O_\nfa$.
	Union and intersection are then computed using the classical NFA construction.
	So, $\varphi \models A$ is decidable by Algorithm~\ref{algoG}
        where acceptors are denoted by NFAs.
	However, acceptors can have $O(|A|^{|\varphi|})$ number of states.
	In fact, the alphabet of any acceptors is already exponential in $|\varphi|$ since letters are tuples whose size is the number of path variables.
	Thus, the call to \texttt{buildAcceptor} at line 21 takes an exponential time in general and a polynomial time if the formula is fixed.
	
	In order to obtain an \textsc{NPSpace} algorithm, we cannot construct explicitly this tuple-acceptor.
	Actually, Algorithm~\ref{algoG} constructs the acceptor only for checking its non-emptiness.
	Moreover, non-emptiness of the product of NFAs can be computed in \textsc{NPSpace}.
	So, in the following we highlight an upper bound on the
        smallest witness of the non-emptiness of the acceptor returned
        by \texttt{buildAcceptor} and based on it, give an
        \textsc{NPSpace} algorithm which decides if there exists such
        a witness.


	First, $\varphi$ is transformed into an equivalent path
        formula thanks to Lemma~\ref{lem:translate} (line 21 of
        Algorithm~\ref{algoG}. We call again $\varphi$ the resulting
        formula. 	Then all disjunctions are removed from
        $\varphi$ in \textsc{NPSpace} by rewriting any sub-formula
        $\varphi_1 \lor \varphi_2$ by $\varphi_i$ where $i$ is
        non-deterministically chosen.
	We obtain $\varphi$ of the form $\bigwedge_{i=1}^k l_i$ where
        each $l_i$ are literals. The function call
        \texttt{buildAcceptor} on $\varphi$ constructs only a product
        of NFA, due to the conjunctive form of $\varphi$.
	So, at line 22 the algorithm decides if $\bigcap_{i=1}^k
        L(B_i) \neq \varnothing$ where each $B_i$ is an NFA
        constructed at line 6 (based on Lemma~\ref{lem:basic}). 
        The size of the NFA resulting from the product of the $B_i$ is 
        $\prod_{i=1}^{k} \dim(B_i)$, which is in
        $O(|A|^{|\varphi|})$. In particular, the predicates of the
        form $\pi\not\in L$ where $L$ is represented by some NFA $N$
        are checking by taking the complement of $N$, causing an
        exponential blow-up in $|\varphi|$ (which takes into account
        the size of $N$), but this blow-up is taken into account in
        the bound $|A|^{|\varphi|}$. Hence, the product is non-empty iff it accepts a
        word of length at most $O(|A|^{|\varphi|})$.


 

        Our \textsc{NPSpace} algorithm guesses such a witness on-the-fly and controls its length using a counter.
	So, only the length and the current state of each NFAs of the product need to be memorised.
	The length can be represented by a binary counter up to
        the value $O(|A|^{|\varphi|})$, so with a size logarithmic in
        $|A|$ and polynomial in $|\varphi|$. 


	The  algorithm goes as follow.
	Initially, the length is set to zero and each state variables are non-deterministically assigned to an initial state.
	At any iteration, the algorithm can non-deterministically take
        a transition if the length counter is small enough or terminates.
	A transition is taken by guessing a letter and assigning each state variable to a possible successor.
	At termination, the algorithm returns if all state variables are assigned to accepting states.
	
	Clearly, the sum of all representation sizes of variables is
        logarithmic in $|A|$ and polynomial in $|\varphi|$.
	In addition, an iteration or the halting can be executed with the same space.
	Thus, the workspace of our algorithm is logarithmic if the formula is fixed and polynomial otherwise.
	


	\emph{Lower bounds} Now, we show the lower bounds.
        Let $A_1, \dots, A_k$ be $k$ DFAs.
        The proof goes by reduction from the problem of deciding $\bigcap_{i=1}^{k} L(A_i)
        \neq \varnothing$, which is known \cite{Galil1976} to be
        \textsc{PSpace-Hard} in general and \textsc{NLogSpace-Hard} if
        $k$ is fixed.
        So, we construct $A$ an NFA as the disjoint union of each $A_i$, i.e $A = A_1 \uplus \dots \uplus A_n$.
        Then we define $\varphi \in \logic_\text{NFA}$ as follows.
        $$
        \exists \pi_1 \colon q_1 \xrightarrow{u} q'_1,
        \dots,
        \exists \pi_k \colon q_k \xrightarrow{u} q'_k,
        \left( \bigwedge_{1 \leq i \leq k}\init(q_i) \land \final(q'_i) \right)
        \land
        \bigwedge_{1 \leq i < j \leq k} q_i \neq q_j
        $$
        The left-hand side part of $\varphi$ asks for $k$ accepting runs on the same input and the right-hand side part of $\varphi$ constrains these paths to start in distinct states.
        By the disjointness of the construction an accepting run in $A$ is an accepting run of some $A_i$.
        In addition, there are exactly $k$ initial states, one of each $A_i$ since the automata are deterministic.
        Thus $A \models \varphi$ if and only if $\bigcap_{i=1}^{n} L(A_i) \neq \varnothing$.
	\qed
    \end{proof}



\subsection{Proof of Theorem~\ref{thm:propNFA}}

We may write $p\rightarrow q$ instead of $p\xrightarrow{u} q$ to mean
that there exists a run from $p$ to $q$, when we do want to capture
the value of $u$. 

An NFA is exponentially ambiguous if for all input words there is at
most an exponential number of accepting runs, iff it does not contain a cycle on
$\epsilon$, iff it does not satisfy the $\logic_\nfa$-formula:
$$
	\begin{array}{l}
	\exists \pi_{1} \colon q_{0} \xrightarrow{\phantom{u}} q_1,\\
	\exists \pi_{2} \colon q_{1} \xrightarrow{u} q_{1},\\
	\exists \pi_{3} \colon q_{1} \xrightarrow{\phantom{u}} q_2,
	\end{array}\
	\init(q_0) \land \final(q_2)\land u=\epsilon
$$



By \cite{DBLP:journals/tcs/WeberS91}, an automaton with output has a
polynomial ambiguity if and only if any input word has at most a
polynomial number (in the size of the word) of accepting runs, iff 
it does not satisfy the pattern of Figure~\ref{fig:ExpAmbiguity},
which is expressible by the $\logic_\nfa$-formula:
$$
	\begin{array}{l}
	\exists \pi_{0, 1} \colon q_{0} \xrightarrow{\phantom{u}} q_1,\\
	\exists \pi_{1, 1} \colon q_{1} \xrightarrow{u} q_{1},\\
	\exists \pi'_{1, 1} \colon q_{1} \xrightarrow{u} q_{1},\\
	\exists \pi_{1, 2} \colon q_{1} \xrightarrow{\phantom{u}} q_2,
	\end{array}\
	\init(q_0) \land \final(q_2)
$$
\begin{figure}
	\centering
	\drawExpAmbiguity
	\caption{Pattern of non polynomial ambiguity}
	\label{fig:ExpAmbiguity}
\end{figure}

By \cite{DBLP:journals/tcs/WeberS91}, an automaton with output have a
constant (in the size of the automaton) number of accepting runs per
input word
(called finite ambiguity) iff it does not satisfy the pattern of Figure~\ref{fig:FiniteAmbiguity}.
This pattern is expressed in $\logic_\nfa$ by:
$$
	\begin{array}{l}
	\exists \pi_{0, 1} \colon q_{0} \xrightarrow{\phantom{u}} q_1,\\
	\exists \pi_{1, 1} \colon q_{1} \xrightarrow{u} q_{1},\\
	\exists \pi_{1, 2} \colon q_{1} \xrightarrow{u} q_2,\\
	\exists \pi_{2, 2} \colon q_{2} \xrightarrow{u} q_{2},\\
	\exists \pi_{2, 3} \colon q_{1} \xrightarrow{\phantom{u}} q_{3},\\
	\end{array}\
	\init(q_0) \land \final(q_3)
$$
\begin{figure}
	\centering
	\drawFiniteAmbiguity
	\caption{Pattern of non finite (constant) ambiguity}
	\label{fig:FiniteAmbiguity}
\end{figure}
\qed



==> app-sum.tex <==
\section{A pattern logic for sum-automata -- Section \ref{sec:sum}}



\begin{lemma} \label{lem:goodsum}
	Parikh automata is an effective good class of tuple acceptors
        for the monoid $\M_\text{Sum} = (\Z,+,0)$ and the set of output
        predicates $\{\leq\}$.
	The size of the PA $P$ for the predicate $t_1\leq t_2$ can be bounded as follows:
	\begin{itemize}
		\item
		the number of states of $P$ is $O(|A|)$
		\item
		the dimension is constant
		\item
		the number of different vectors occurring on
                transitions and the maximal absolute value occurring
                in vectors are constant if weights of $A$ are unary encoded and $O(|A| \times \sum_{i=1}^{\alpha(p)}|t_i|)$ if the encoding is in binary
		\item
		the acceptance Presburger formula is constant
	\end{itemize}
\end{lemma}
\begin{proof}
	We show that the Parikh automata fulfils the properties of a good class.
	\begin{enumerate}
	\item[\ref{goodreg}.]
		The property holds for PA, as a generalisation of NFA.
	\item[\ref{goodout}.]
		Consider the automata with output $A \in
                \trs(\M_\suma)$ with a set of states $Q$ and a
                (finite) set of output values $D_f \subset \Z$
                occurring on its transitions.
		Let take also $X = \{ \pi_1, \dots, \pi_n \}$ a finite ordered set of path variables of cardinal $n$.
		We describe the construction of a tuple acceptor for $t_1 \leq t_2$ with $t_1, t_2 \in \text{Terms}(X, \cdot, \varepsilon)$.
		We fix $t_i = \pi_{i, 1} \dots \pi_{i, n_i}$ with $i \in \{1, 2\}$.
		This predicate is true if and only if $\sum_{j=1}^{n_1} \out(\pi_{1, j}) \leq \sum_{j=1}^{n_2} \out(\pi_{2, j})$.
		However, the PA that we construct takes $\pi_1 \conv \dots \conv \pi_n$ as input word.
		So, for all $i \in \{1, 2\}$ the PA uses a counter $c_i$ to compute the value $\sum_{j=1}^{n} \out(\pi_{1, j}) \times k_{i, j}$ where $k_{i, j}$ is the number of occurrences of $\pi_j$ in $t_i$.
		Then the resulting PA $P$ accepts if $c_1 \leq c_2$. If the weights
                of $A$ are encoded in unary, then by splitting the
                transitions of $P$, we can assume that its increments
                are in $0,1$. 

                The resulting PA for $t_1 \leq t_2$ has:
			\begin{itemize}
			\item
				if weights of $A$ are encoded in binary
				\begin{itemize}
					\item a constant dimension.
					\item a constant number of states.
					\item a maximal absolute value appearing in vectors at most $\log(\ell) \times (n_1 + n_2)$ where $\ell$ is the maximal absolute value of $D_f$.
					\item a number of different vectors at most $(|D_f| \times (n_1 + n_2))^2$.
				\end{itemize}
			\item
				if weights of $A$ are encoded in binary
				\begin{itemize}
					\item a constant dimension.
					\item a number of states in $O(|A|)$.
					\item a constant maximal absolute value appearing in vectors.
					\item a constant number of different vectors.
				\end{itemize}
			\end{itemize}
	\item[\ref{goodneg}.]
		We are able to construct a tuple acceptor for $t_1 <
                t_2$ as above but with $c_2 < c_1$ as acceptance condition.
	\item[\ref{goodclos}.]
		Parikh automata are closed by union and intersection \cite{10.1007/3-540-45061-0_54}.
		Those operations can be realise in \textsc{PTime}.
	\end{enumerate}
\end{proof}

\subsection{Proof of Theorem~\ref{thm:PLsum-complexity}}

\begin{proof}
    \textbf{The logic $\logic_\suma$} Consider first the logic $\logic_\suma$. The algorithms are
   similar to the case of finite automata and transducers. As for
   transducers, it boils down to checking the emptiness of a product
   of Parikh automata, whose basic blocks are constructed thanks to
   Lemma~\ref{lem:goodsum}.  The \textsc{PSpace} upper bound is guaranteed
   thanks to the short witness property of
   Lemma~\ref{lem:witness}. The \textsc{PSpace} lower bound is
   obtained via the same proof as for NFA. 


   To get the NP upper bound in the case where the formula is fixed,
   similarly to the transducer case, the Parikh automaton $P$
   corresponding to the product of the Parikh automata for the atoms 
   has polynomial size. However, unlike in the transducer case,
   and although the Presburger formula for the acceptance condition of
   $P$ is
   constant, as well as the dimension, the values occurring in the
   vectors of $P$ are not unary encoded, because they correspond to
   values of the sum-automata $A$ which is model-checked, and which
   are themselves encoded in binary. Theorem~\ref{thm:parikh} ensures
   that in that case non-emptiness can be tested in \textsc{NP}. 




	% We start by showing the upper bounds.
	% Let set $\psi \in \logic_\text{Sum}$ a pattern formula and $A$ a sum-automaton.
	% % This proof, present an algorithm which decide $\varphi \models A$ in \textsc{NPSpace} which became in \textsc{NLogSpace} if the formula is fixed and in addition the values of the automaton are encoded in unary.
	% We provide an other algorithm, in \textsc{NP-C}, when the formula is fixed but the values of the automaton are encoded in binary.
	
	% Following Lemma~\ref{lem:goodsum}, the model-checking problem is decidable by Algorithm~\ref{algoG} which construct a PA of size $O(|A|^{|\varphi|})$.
	% Thus, to obtain \textsc{PSpace}-membership we cannot construct explicitly this automaton.
	% Actually, Algorithm~\ref{algoG} construct the acceptor only for checking its non-emptiness.
	% % Then, in the following we highlight an upper bound on the smallest witness of the non-emptiness of the acceptor returned by \texttt{buildAcceptor} and base non it, give an \textsc{NPSpace} algorithm which decides if there exists such a witness.
	
	% We start by considering w.l.o.g a special form of the pattern formula $\varphi$ constructed by Algorithm~\ref{algoG} at line 16.
	% We can remove all disjunctions of $\varphi$ in \textsc{NPSpace} by rewriting any sub-formula $\varphi_1 \lor \varphi_2$ by $\varphi_i$ where $i$ is non-deterministically chosen.
	% We obtain $\varphi$ of the form $\bigwedge_{i=1}^{m} r_i \land \bigwedge_{j=1}^{k} s_j$ where each $r_i$ are non-output literals and each $s_j$ are output literals.
	% Thus, the function \texttt{buildAcceptor} realise only product of PAs, due to the conjunctive form of $\varphi$.
	% So, at line 19 the algorithm decides if $\bigcap_{i=1}^{m} L(B_i) \cap \bigcap_{j=1}^{k} L(P_j) \neq \varnothing$ where
	% each $B_i$ is an NFA, constructed whether at line 4 using using Lemma~\ref{lem:basic} and
	% each $P_j$ is a PA constructed at line 2 using Lemma~\ref{lem:goodsum}.
	% Note that, each $B_i$ can be seen as PAs with dimension zero.
	
	% Now, we give an \textsc{NPSpace} algorithm which decides the non-emptiness of the product.
	% Let denote $d_j, \alpha_j$ and $\ell_j$ the dimension, the number of different vectors occurring on transitions and the maximal absolute value appearing in vectors of $P_j$.
	% We define also, $d = \sum_{j=1}^{k} d_j$, $\alpha = \sum_{j=1}^{k} \alpha_j$, $\ell = \max_{j = 1}^{k} \ell_j$ and $s = \prod_{j=1}^{k}\dim(P_j) \times \prod_{i=1}^{m}\dim(B_i)$.
	% With Lemma~\ref{lem:witness}, we can ensure that the size of a smallest witness for the non-emptiness is at most exponential in $d, \alpha$ and polynomial in $\ell, s$.
	% By Lemma~\ref{lem:goodsum}, $d$ is constant and $\alpha, \ell$ are $O(|A| \times |\varphi|)$ if weighs of $A$ have a binary encoding and constant is the encoding is in unary.
	% Furthermore, $s$ is $O(|A|^{|\varphi|})$.
	% Thus, the size of a smallest witness is $O(2^{|A| \times |\varphi|})$ in general and $O(|A|)$ if the formula is fixed and weights of $A$ are encoded in unary.
	
	
	
	
	
	% Intuitively, our algorithm guesses such a witness on-the-fly and controls its length using a counter.
	% Our algorithm need to memorised the length and the current state of each PAs of the product.
	% The length can be represented by a binary counter and the current states can be represented by $k+m$ variables with a range of size $s$.
	% We also need $d$ binary counters to maintain the values computed by PAs, which cannot be bigger than $\ell$ times the length of the witness.
	% Our algorithm goes as follow.
	% Initially, the length is set to zero and each state variables are non-deterministically assigned to an initial state.
	% At any iterations, the algorithm can non-deterministically takes a transition if the length counter is small enough or terminates.
	% A transition is taken by guessing a letter and assigning each state variables to a possible successor.
	% At termination, the algorithm accept if all state variables are assigned to accepting states and Presburger formula of acceptance of each PAs are satisfy.
	% Since those formula are fixed then they satisfiability we can decide in \textsc{NLogSpace} by Theorem~6~(A) of \cite{scarpellini}.
	
	% Clearly, the sum of the representation size of variables is $O(|A| \times |\varphi|)$ in general and $O(\log(|A|))$ if the formula is fixed and weights of $A$ are encoded in unary.
	% In addition, an iteration or the halting can be executed with the same space.
	% Thus, the workspace of our algorithm is logarithmic if the formula is fixed and polynomial otherwise.
	
	% Finally, we show the \textsc{NP} upper bound when the formula is fixed.
	% In this condition, the product can be effectively constructed in polynomial time.
	% So, we construct $P$ the PA defined as $\bigcap_{i=1}^{m} B_i \cap \bigcap_{j=1}^{k} P_j$.
	% By Lemma~\ref{lem:goodsum}, $d, \alpha, \ell$ and $s$ are $O(|A|)$.
	% Applying Theorem~\ref{thm:parikh}, we can decide the emptiness of $P$ in \textsc{NP}.
	
   For the \textsc{NP} lower bound, we reduce the \textsc{NP-c} \emph{Set Partition}
   problem, which asks, given a multi-set $S = {x_1, . . . , x_k}$ of
   natural number, whether there exists $I$ such that $\sum{i\in I}
   x_i =  \sum_{i\not\in I} x_i$. One construct the sum-automaton of
   Figure~\ref{fig:np} and the following $\logic_{Sum}$ formula:
	$$
	\exists \pi_1:q_0\xrightarrow{v_1} q_f,
	\exists \pi_2:q_f\xrightarrow{v_2} q_f,
	\init(q_0) \land \final(q_f) \land v_1 = v_2
	$$
	The reduction is linear because the automata construction is
        linear and the formula is constant.
	\begin{figure}[!h]
		\centering
		\drawNP\\
		\caption{Sum-automaton used for encoding Set Partition}
		\label{fig:np}
	\end{figure}


\vspace{2mm} \textbf{The logic $\logic_\suma^{\neq}$}
	We finally focus here on the logic
        $\logic^{\neq}_\suma$. Membership to \textsc{PSpace} is
        immediate as it is a fragment of $\logic_\suma$. Also,
        \textsc{PSPace}-hardness still holds since our reduction of
        the intersection emptiness of DFA does not
        need output predicates. 


        
        Now, we consider that the formula is
        fixed and show that the model-checking problem is in
        \textsc{PTime}. 	We can assume that the formula is
        without disjunction as it can be put in disjunctive normal
        form at constant cost (the formula being fixed) and each
        disjunct can be treated separately. 
	Also, we translate the formula into the intermediate
        syntax by Lemma~\ref{lem:translate} and obtain a path
        formula over some set of variables $\{ \pi_1, \dots, \pi_n
        \}$. It is necessarily of the form $\varphi = \bigwedge_{i=1}^{m} r_{i }\land \bigwedge_{j=1}^{m'} s_{j}$
	where the $r_{i}$ are input, path and state literals,  and the $s_j$
        are output literals.



	Let $A$ be a sum-automaton, we now provide a \textsc{PTime}
        procedure for deciding if $\varphi \models A$. This algorithm
        makes use of the \textsc{PTime} procedure to decide
        $k$-valuedness of a sum-automaton for a fixed
        $k$~\cite{DBLP:conf/fsttcs/FiliotGR14}.
 

        First, by Lemma~\ref{lem:basic} we can construct $N$ an NFA
        which verifies the constraints $r_i$. It has polynomial size
        in $A$ and $\varphi$ since the formula is fixed. 


	Second, we explain how to treat output constraints. To
        simplify the proof, we first assume that they are of the form 
        $s_{j} = \pi_x \neq \pi_y$ where $\pi_x,\pi_y$ are path
        variables (and not general terms). The extension to terms is
        technical but not difficult. We define $A_{j}$ as a sum-automaton which maps $\pi_1 \conv \dots \conv \pi_n$ to $A(\inp(\pi_x)) - A(\inp(\pi_y))$.
	We construct $A_j$ from the product $A^n$ where each
        transition label $v\in\Z^n$ are replaced by the integer value
        $v[x] - v[y]$. Note that, 
        $A_j(\pi_1\otimes \dots \otimes \pi_n)=0$ iff $s_{j} =
        \pi_x\neq \pi_y$ does not hold.
	Then, we construct $A'$ a sum-automaton which non-deterministically chooses $j \in \{ 1, \dots, m \}$ and runs $N \times A_j$.
        We have that $A\models \varphi$ iff there exists $\pi_1\otimes
        \dots \otimes \pi_n$ such that $\pi_1\otimes\dots \otimes
        \pi_n\in L(N)$ and $0\not\in R_{A'}(\pi_1\otimes \dots \otimes
        \pi_n)$ (the set of values associated with $\pi_1\otimes \dots \otimes
        \pi_n$ by $A'$).


        In order to check the latter, we compute the minimum $k$ such
        that $A'$ is $k$-valued but not $(k-1)$-valued. This can be
        done in \textsc{PTime} thanks to
        \cite{DBLP:conf/fsttcs/FiliotGR14} (because the valuedness is
        at most $n^2$ which is fixed, so we can use an iterative
        algorithm). Once the valuedness $k$ of $A'$ is known, it
        suffices to add to $A'$ a disjoint part which always associate
        the value $0$ to any product $\pi_1\otimes \dots \otimes
        \pi_n$ in $L(N)$ (by adding a copy of $N$ with value $0$ on
        all transitions). We call $A''$ the resulting sum-automaton. 
        Clearly, $0\in  R_{A''}(\pi_1\otimes \dots \otimes \pi_n)$ for
        all $\pi_1\otimes \dots \otimes \pi_n\in L(N)$. We know that
        $A''$ is $(k+1)$-valued, but it could be also $k$-valued, in
        the case where $0\in  R_{A'}(\pi_1\otimes \dots \otimes \pi_n)$ for
        some $\pi_1\otimes \dots \otimes \pi_n\in L(N)$. In other
        words, $A\not\models \varphi$ iff $A''$ is $k$-valued, which
        again can be tested in
        \textsc{PTime}~\cite{DBLP:conf/fsttcs/FiliotGR14}.

        
        To extend this algorithm to constraints $s_j = t_x\neq t_y$
        with terms, we follow similar ideas as before. In particular,
        to construct $A_j$, the values of any tuple $v\in\Z^n$
        occurring on a transition of $A^n$ is replaced by 
        $\sum_{i=1}^n v[i].(k_{x,i}-k_{y,i})$ where $v[i]$ is the
        $i$th value of $v$, $k_{x,i}$ (resp. $k_{y,i}$) is the number of occurrences of
        $\pi_i$ in $t_x$ (resp. $t_y$). 
	\qed
\end{proof}



\subsection{Proof of Theorem~\ref{thm:propsum}}

By \cite{DBLP:conf/fossacs/DaviaudJRV17}, a sum-automaton is
$k$-sequential if and only if (as a direct encoding of the definition
of \cite{DBLP:conf/fossacs/DaviaudJRV17}) it does not satisfy the following
$\logic_\suma^\neq$-formula, where the general form of the pattern is
depicted on Figure~\ref{fig:BTP}:
$$
\begin{array}{l}
\exists_{i = 1}^{k} \exists_{j=0}^{k} \pi_{i,j} \colon q_{i-1, j} \xrightarrow{u_{i, j} \mid v_{i, j}} q_{i, j},\\
\exists_{i = 1}^{k} \exists_{j=0}^{k} \pi'_{i,j} \colon q_{i, j} \xrightarrow{u'_{i, j} \mid v'_{i, j}} q_{i, j},
\end{array}
 \bigwedge_{j \neq j'} \bigvee_{i = 1}^{k} \bigwedge_{i' = 1}^{i} \bigwedge
\begin{cases}
	u_{i', j} = u_{i', j'} \\
	u'_{i', j} = u'_{i', j'} \\
	v'_{i, j} \neq v'_{i, j'}
\end{cases}
$$




==> app-trans.tex <==
\section{Parikh Automata}

For the transducer and sum-automata logic, getting decidability relies
on the fact that Parikh automata can be used as acceptors for tuples
of paths. We make clear here what we mean by Parikh automata and state
a few properties we need. 


Acceptance conditions of Parikh automata are given by (existential)
Presburger formulas, i.e. formulas of the form $\exists x_1\dots
\exists x_n \phi$ where $\phi$ is a quantifier-free first-order
formula built over any constant $n\in\N$, the addition $+$ and
comparison $<$. 

\begin{definition}
    A Parikh automaton of dimension $d$ over some alphabet $\Lambda$ is pair $P = (A,\zeta)$  where
    $A$ is an automaton over $\Lambda$ with outputs
    in the monoid $(\N^d, +_{\N^d}, 0_{\N^d})$, and $\zeta$ is an
    existential Presburger formula with $d$ free variables. 
\end{definition}

The language $L(P)$ defined by $P$ is the set of words $u\in\Lambda^*$ such that there exists $v\in\N^d$ such that $(u,v)\in \sem{A}$ and $v\models \zeta$.
The representation size of $P = (A, \zeta)$ a Parikh automaton of
dimension $d$ where $A=(Q, I, F, \Delta, \gamma)$ is defined as $|P| =
|\zeta| + |Q| + (d\log(\ell)+1)|\Delta|$ with $\ell$ is the maximal
absolute value appearing on a vector of a transition, and $|\zeta$ is
the number of symbols in $\zeta$ plus the size (in binary) of the
constants in $\N$ it contains. 


The non-emptiness problem consists in deciding whether $L(P) \neq
\varnothing$.


% ----------------------------------------------------------------------- %


\begin{theorem} \label{thm:parikh}
    The non-emptiness problem is \textsc{NPTime-C} for Parikh automata.
    It is in \textsc{NLogSpace-C} if the dimension and Presburger formula are fixed, and the vector values are encoded in unary. 
\end{theorem}

Hardness is easily obtained by encoding subset sum, and actually holds
even if the dimension is restricted to $1$ and the Presburger formula
is as simple as $x=0$. 


% It heavily exploits the fact that numbers
% are encoded in unary. To the best of our knowledge, no polynomial time
% subclass of Parikh automata is known to have \textsf{PTime} complexity
% when the numbers are encoded in binary. By restricting the class of
% Presburger acceptance formulas to formulas that do not test for
% equality, we obtain such a class.

% Formally, a equality-free Presburger formula is a disjunction of
% conjuncts of atoms of the form $x<y$, $x\neq y$ and $0<x$. 


% \begin{theorem}
    % The non-emptiness problem is in \textsf{PTime} for Parikh automata whose acceptance
    % conditions are given by equality-free Presburger formulas. 
% \end{theorem}
% Note that it is not required that the vector dimension is fixed. 
% \begin{proof}
    % We rely on the result of \cite{} which states that deciding the
    % existence, in a $\mathbb{Z}^k$-weighted directed graph $G$, of a cycle
    % whose weights sum to $0$ on all dimensions can be done in
    % \textsf{PTime} (even if $k$ is not fixed). Such a cycle is called
    % a $0$-cycle.


    % First, as for instance proved in~\cite{}, the latter result can be
    % used to show that the following problem on graphs $G$ can be
    % decided in polynomial time. Given two sets of vertices $S,T$, are there
    % $s\in S$ and $t\in T$ such that there exists a path from $s$ to
    % $t$ with strictly positive accumulated weights on all dimensions. 

    
    % Let us briefly recall how the algorithm works, for $S=\{s\}$ and
    % $T=\{t\}$ (otherwise, it suffices to iterate on all pairs
    % $(s,t)\in S\times T$). The graph $G$ is transformed into $G'$ of
    % dimension $k+1$ obtained by adding to $G$:
% \begin{enumerate}
  % \item an extra vertex $u$ with a $(0,\dots,0,-1)$-valued loop
  % \item a $(-1,\dots,-1)$-valued edge from $t$ to $u$
  % \item $k$ loops on $t$ valued respectively by
    % $(0,\dots,0,-1,0,\dots,0,+1)$ where $-1$ is at the $i$th dimension
    % for all $i=1,\dots,k$
  % \item a $(0,\dots,0)$-valued edge from $u$ to $s$
  % \item the weight $(x_1,\dots,x_k)$ of any edge in $G$ is replaced by
    % the weight $(x_1,\dots,x_k,+1)$. 
% \end{enumerate}

% It can be shown that there exists a $0$-cycle in $G'$ iff there exists
% a strictly positive path from $s$ to $t$ in $G$. Briefly, the
% dimension $k+1$ enforces any $0$-cycle to visit $s$, $t$ and
% $u$. Since going from $t$ to $u$ decreases every dimension of $1$, it
% must be the case that there exists a strictly positive path from $s$
% to $t$ if there is a $0$-cycle in $G'$. 



% Now, suppose that we are given a Parikh automaton $P=(A,\zeta)$ with acceptance
% given by some equality-free Presburger formula $\zeta = \bigvee_{j=1}^m \zeta_j$
% where each $\zeta_i$ is a conjunction of atoms of the form $x_i<x_j$,
% $x_i\neq y_i$ and $0<x_i$, where $x_i$ denotes the $i$th vector
% dimension. We provide a PTime algorithm for the case where $m=1$. If
% $m>1$, it suffices to run on the $m$ formulas $\zeta_j$ respectively
% as long as the answer is negative. 


% Now, $A$ is transformed into a directed graph of dimension 

% \end{proof}


We now turn to the non-emptiness problem of the intersection of $k$
languages defined by Parikh automata. This problem was shown to be
\textsc{PSpace-Complete} in \cite{DBLP:conf/lics/FigueiraL15}. A careful analysis of the
proof allows us to obtain a small witness property:

\begin{lemma} \label{lem:witness}
    Given $k$ Parikh automata $P_i = (A_i,\zeta_i)$ over some
    (unfixed) alphabet $\Lambda$, each of which has dimension
    $d_i$, $n_i$ states and $\alpha_i$ different vectors occurring on
    its transitions. Let $\ell$ be the maximal absolute value occurring
    on a vector of the $P_i$ for all $i$. 

    Then $\bigcap_{i=1}^k L(P_i)\neq
    \varnothing$ iff there exists $u\in \bigcap_{i=1}^k L(P_i)$ such that 
    the length of $u$ is exponential in $\sum_i d_i + \sum_i \alpha_i$ and
    polynomial in $n_1\times\dots\times n_k$ and $\ell$. 
\end{lemma}

% In the latter lemma, the size of the alphabet $\Lambda$ does not play
% any role in the size of a short witness. Also note that $\ell$ being
% encoded in binary, the witness has exponential length with respect to 
% the size of $\ell$. 


% \red{
	% \begin{lemma} \label{lem:witness}
		% Given an unfixed alphabet $\Sigma$.
		% % Given $k$ Parikh automata $P_i = (A_i,\zeta_i)$ over $\Sigma$ each of which has dimension $d_i$, $n_i$ states and $\alpha_i$ different vectors occurring on its transitions.
		% Let $\ell$ be the maximal absolute value occurring on a vector of the $P_i$ for all $i$. 
		% Given $k'$ NFA $N_1,\dots,N_k$ over $\Sigma$ each of which has $n'_i$ states.
		
		% Then $\bigcap_{i=1}^k L(P_i) \cap \bigcap_{i=1}^{k'} L(N_i) \neq
		% \varnothing$ iff there exists $u\in \bigcap_{i=1}^k L(P_i) \cap \bigcap_{i=1}^{k'} L(N_i) $ such that 
		% the length of $u$ is exponential in $\sum_i d_i + \sum_i \alpha_i$,
		% polynomial in $n_1\times\dots\times n_k$, $n'_1\times\dots\times n'_{k'}$ and $\ell$.
	% \end{lemma}
% }


% ----------------------------------------------------------------------- %


% \begin{corollary} \label{cor:parikh}
    % Given $k$ Parikh automata $P_i = (A_i,\zeta_i)$ over some
    % (unfixed) alphabet $\Lambda$ and $m$ NFA $B_1,\dots,B_m$, it is
    % decidable in \textsc{PSpace} whether 
    % $$
    % \bigcap_{i=1}^k L(P_i)\cap \bigcap_{i=1}^m \overline{L(B_i)} \neq \varnothing
    % $$
% \end{corollary}
% \begin{proof}
    % By Savitch's theorem, we only have to exhibit an non-deterministic
    % algorithm running in polynomial space (in the $P_i$ and the
    % $B_i$). By the previous result, applied on the $P_i$ and the DFA
    % obtained $A_i$ from the $B_i$ by subset construction (which are as well
    % Parikh automata of dimension $0$), the above intersection is
    % non-empty iff there exists a witness of size exponential in the
    % size of the $P_i$ and the $B_i$. 


    % Hence, the non-deterministic algorithm guesses such a witness
    % on-the-fly (using a counter up to an exponential value,
    % polynomially represented in binary, to control its length), and
    % apply a product construction on the $P_i$ and the $A_i$ (which do
    % not need to be explicitly constructed, and whose transitions can
    % be evaluated in polynomial time). Eventually, the vector values
    % induced by this witness is tested against the Presburger
    % formulas, whose satisfiability can also be checked in polynomial
    % space. \qed
% \end{proof}


% ----------------------------------------------------------------------- %


\section{A pattern logic for transducers -- Section
  \ref{sec:transducers}}

\subsection{Undecidability -- Proof of Theorem~\ref{thm:undec}}

\begin{proof}
    We encode the Post Correspondence Problem (PCP). Given a
    set of dominos $\{(u_1,v_1),\dots,(u_n,v_n)\}$ over some alphabet
    $\Sigma$, we construct the transducer $T_{pcp}$ of
    Figure~\ref{fig:pcp}, which defines  the following subset of
    $\{1,\dots,n\}^*\times \Sigma^*$: $\{ (i_1\dots i_k,u_{i_1}\dots
    u_{i_k})\mid i_j\in\{1,\dots,n\}\}\cup 
\{ (i_1\dots i_k,v_{i_1}\dots
    v_{i_k})\mid i_j\in\{1,\dots,n\}\}$. Then, this instance has a
    solution iff there exists two different accepting paths over the
    same input and output words, iff the following
    $\logic[\varnothing]$ is satisfied by $T_{pcp}$:
	$$
		\varphi_{pcp} =
			\exists \pi \colon q \xrightarrow{u \mid v} q,
			\exists \pi' \colon q' \xrightarrow{u \mid v} q',
			q \neq q'
	$$
	% We show the undecidability of $T_{pcp} \models \varphi_{pcp}$ by reduction from the Post correspondence problem.
	% Given two finite lists $u_1, \dots, u_n$ and $v_1, \dots, v_n$ of finite words over a non-unary alphabet.
	% % The solution of the Post correspondence problem is a finite sequence $x_1, \dots, x_N$ where each $x_i$ are in $\{1, \dots, n\}$ such that $u_{x_1} \dots u_{x_N} = v_{x_1} \dots v_{x_N}$.
	% So, the formula ask if there exists two distinct loop on the come input word $x_1 \dots x_N$ which produce the same output word.
	% Clearly, the formula is satisfy if and only if $x_1, \dots, x_N$ is solution of the Post correspondence problem.
		\begin{figure}[h!]
			\centering
			\drawPcp
			\caption{The transducer $T_{pcp}$ which is non-deterministic}
			\label{fig:pcp}
		\end{figure}
	\qed
\end{proof}


\subsection{Parikh Automata Form a Good Class}

We define the set of output predicates 
$\O_{trans} = \{ \not\prefix, \in N, \not\in N, \leq, <\}$, for any $N$ regular language over
$\Gamma$ (assumed to be represented by some NFA).


\begin{lemma} \label{lem:goodtrans}
	Parikh automata (PA) is an effective weakly good class of tuple
        acceptors for any free monoid and the set of output predicates
        $\O_{Trans}$.
	The size of the PA for the predicates of $\O_{Trans}$ can be bounded as follows (taking the notations of
        Condition~\ref{goodout} of the definition of good class):
	\begin{itemize}
		\item the number of states is $O(|A|^{n})$ and
                  $O(|A|^{n \times |N|})$ for the membership
                  predicates, where $N$ is an NFA representing the
                  regular language used in the predicate.
		\item the dimension is $O(\sum_{i=1}^{\alpha(p)}|t_i|)$
		\item the maximal absolute value occurring in vectors is $O(\log(|A|) \times \sum_{i=1}^{\alpha(p)}|t_i|)$
		\item the number of different vectors occurring on transitions is $O(\log(|A|) \times \sum_{i=1}^{\alpha(p)}|t_i|)$
		\item the acceptance Presburger formula is constant
	\end{itemize}
\end{lemma}
\begin{proof}
We show that the Parikh automata fulfils the properties of a good class.
\begin{enumerate}
\item[\ref{goodreg}.]
	The property holds for PA as a generalisation of NFA.
\item[\ref{goodout}.]
	Consider the automata with output $A \in \trs(\M_\trans)$ with a set of states $Q$ and a (finite) set of output values $D_f \subset \Gamma^*$ occurring on its transitions.
	Let take also $X = \{ \pi_1, \dots, \pi_n \}$ a finite ordered set of path variables of cardinal $n$.
	Now we describe the construction of a tuple acceptor for each atom of $\O_\trans$ as follows:
	\begin{itemize}
	\item 
		$|t_1| \preceq |t_2|$ with $t_1, t_2 \in \text{Terms}(X, \cdot, \varepsilon)$ and where $\preceq\ \in \{\leq, <\}$.
		We fix $t_i = \pi_{i,1} \dots \pi_{i, n_i}$ with $i \in \{1, 2\}$.
		The predicate $|t_1|\preceq |t_2|$ is true if and only if
		$\sum_{j=1}^{n_1} |\out(\pi_{1,j})| \preceq \sum_{j=1}^{n_2} |\out(\pi_{2,j})|$.
		However, the PA that we construct takes $\pi_1 \conv \ldots \conv \pi_n$ as input word.
		So, for all $i \in \{1, 2\}$ the PA uses the counter $c_i$ to compute the value $\sum_{j=1}^{n} |\out(\pi_i)| \times k_{i, j}$ where $k_{i, j}$ is the number of occurrences of $\pi_j$ in $t_i$.
		Then the PA accepts if $c_1 \preceq c_2$.
		
		Furthermore, there exists a PA which decides if $|t_1|\preceq |t_2|$ with:
		\begin{itemize}
			\item A constant number of states.
			\item A constant number of dimensions.
			\item A maximal absolute value appearing in vectors in $O(\log(\ell) \times (n_1 + n_2))$ where $\ell$ is the maximal length of words in $D_f$.
			\item A number of different vectors in $O((\ell \times (n_1+n_2))^2)$.
		\end{itemize}
	
	\item 
		$t\Subset N$ with $t \in \text{Terms}(X, \cdot, \varepsilon)$, $\Subset\ \in \{\in, \not\in\}$ and where the language $N$ is denoted by the NFA $B$ over $\Gamma$.
		We fix $t = \pi'_{1} \dots \pi'_{m}$.
		The predicate $t \in N$ is true if there exists a $m+1$-tuple of state $(q_0, \dots, q_m)$ such that there exists a path in $B$ from $q_{i-1}$ to $q_i$ over the input $\inp(\pi'_i)$ and $q_0$ initial, $q_m$ final.
		However, the PA that we construct takes $\pi_1 \conv \ldots \conv \pi_n$ as input word.
		So, $i\in\{ 1, \dots, n \}$ using the classical product of automata theory we define the NFA $B_i$ as $B^{k_i}$ where $k_i$ is the number of occurrences of $\pi_i$ in $t$.
		Then we construct $\bigconv_{i=1}^{n} B_i$.
		Note that, $t \not\in N$ can be denoted by $t \in \overline{N}$.
		
		Furthermore, there exists a PA which decides if $t\Subset N$ with:
		\begin{itemize}
			\item A constant number in $O(|A|\times 2^{n\times |N|})$.
			\item A constant number of dimensions.
			\item A constant maximal absolute value appearing in vectors.
			\item A constant number of different vectors.
		\end{itemize}
	
	\item 
		$t_1\not\prefix t_2$ where $t_1, t_2 \in \text{Terms}(X, \cdot, \varepsilon)$.
		We fix $t_i = \pi_{i,1} \dots \pi_{i, n_i}$ with $i \in \{1, 2\}$.
		Remark, if $|t_1| \not\leq |t_2|$ then $t_1\not\prefix t_2$ is false.
		Thus, we assume w.l.o.g. that $|t_1| \leq |t_2|$ (it
                has been already shown how to construct PA which check
                this predicate as well as its negation). Under this
                hypothesis, it remains to construct a PA which check
                the existence of mismatch position $\beta$  in $t_1$ and $t_2$, i.e. a
                position in the output they define with different
                labels. Let $Y$ be the set of path variables occurring
                in $t_1$ and $t_2$. The PA reads (convolutions) of
                tuples of paths in $Y$. The position $\beta$ may not
                occur at the same position in the input read by the
                PA, and that is why we need to use counters to
                identify a position $\beta_1$ in the output defined by
                $t_1$, and a position $\beta_2$ in the output defined
                by $t_2$, remember the corresponding output labels (in
                the state of the PA), and later on check that they
                differ, and that $\beta_1=\beta_2$ (using an accepting
                Presburger formula). The way the positions
                $\beta_1,\beta_2$ are chosen by the PA works as
                follows: it guesses an index $i_1\in\{1,\dots,n_1\}$
                and an index $i_2\in\{1,\dots,n_2\}$, intended to
                verify the existence of a mismatch position in the
                output of $\pi_{1,i_1}$ and $\pi_{2,i_2}$. The
                counters will respectively count the length of the
                output produced on $\pi_{1,1}\dots \pi_{1,i_1-1}$ and 
                $\pi_{2,1}\dots \pi_{2,i_2-1}$ (when processing the
                whole tuple of paths), and also the length of the
                output produced in respectively $\pi_{1,i_1}$ and
                $\pi_{2,i_2}$ up to some point non-deterministically
                chosen. 


                The formal construction is very technical but not
                difficult, and overall it yields a PA to check
                $t_1\not\prefix t_2$ with:
		\begin{itemize}
			\item A number of states in $O(n_1 + n_2)$.
			\item A number of dimensions in $O(1)$.
			\item A maximal absolute value appearing in vectors in $O(\log(\ell) \times (n_1 + n_2))$ where $\ell$ is the maximal length of words in $D_f$.
			\item A number of different vectors in $O((\ell \times (n_1+n_2))^2)$.
		\end{itemize}
	\end{itemize}
	\item[\ref{goodclos}.]
		Parikh automata are closed by union and intersection \cite{10.1007/3-540-45061-0_54}.
		Those operations can be realised in
                \textsc{PTime}.\qed
\end{enumerate}
\end{proof}

% % % % % % OLD PRECISE PROOF
%\begin{proof}
%	We show that the Parikh automata fulfils the properties of a good class.
%	\begin{enumerate}
%	\item[\ref{goodreg}.]
%		NFAs can be compiles in Parikh automata of dimension zero.
%	\item[\ref{goodclos}.]
%		Parikh automata are close by intersection and union.
%		\red{Continue... (the cost is +1 dimension and +1 state)}
%	\item[\ref{goodout}.]
%		Now we describe the construction of a path-acceptor for each atom of $\O_{Trans}$ and it negation.
%		We fix the automata with output $A \in \trs(\M_{Trans})$ with a set of states $Q$ and a (finite) set of output values $D_f$ occurring on its transitions.
%		Let take also $X = \{ \pi_1, \dots, \pi_n \}$ a finite ordered set of path variables of cardinal $n$.
%		
%		Assume that for any $v \in D_f$ we have the value $|v|$ which is the number of output letters that the data contain.
%		Also we need for each position $1 \leq p \leq |v|$ the output letter $v[p] \in \Gamma$ which is the $p$th letter of the data $v$.
%		Those values are computable in linear time of $|A|$.
%		\begin{itemize}
%		\item 
%			Predicate $\leq$ of arity two.
%			Consider $t_1, t_2 \in \text{Terms}(X, \cdot, \varepsilon)$.
%			We describe the construction of $P_\leq$ a Parikh automaton of two dimensions which accept the convolutions of $n$ paths of $\paths(A)$ such that $|\out(t_1)| \leq |\out(t_2)|$.
%			The parikh automaton $P$ is define with a single state, initial and final.
%			When, it read a tuple of data, let say $(v_1, \dots, v_n)$, then $P$ increase the dimension $i$ of $\sum_{j=1}^{n} |v_j| \times |t_i|_j$ where $|t_i|_j$ is the number of occurrences of $\pi_j$ in $t_i$.
%			Clearly, at the end of the run the dimension $i$ is equal to $|\out(t_i)|$.
%			So, we filter the acceptance with the Presburger definable constraint $c_1 \leq c_2$.
%			Moreover, we are able to realise the negation of this predicate with the acceptance constraint $c_1 < c_2$.
%		
%			Note that, the dimension and the number of states is constant.
%			The maximal absolute value appearing in vectors is $O(\log(\ell) \times \max_{i=1}^{2}|t_i|)$ where $\ell$ is the maximal length of output string in $D_f$ and $|t_i| = \sum_{j=1}^{n}|t_i|_j$.
%			We deduce that, the number of different vector is $O((\ell \times \max_{i=1}^{2}|t_i|)^2)$.
%		\item 
%			Predicate $\in N$ of arity one where the language $N$ is denoted by the NFA $B$ over the alphabet $\Gamma$.
%			Consider $\pi \in X$.
%			We describe the construction of $P_\in$ a NFA which accept the convolutions of $n$ paths of $\paths(A)$ such that $|\out(\pi)| \in L(B)$.
%			We construct $P_\in$ as a copy of $B$ where we merge letter by letter transitions to obtain transitions labelled by data.
%			Furthermore, we add a self loop reading symbols of $\Lambda \cup Q$ on each states in order to read path of $A$.
%			Moreover, we are able to realise the negation of this predicate with the complement $\overline{N}$ of the language $N$.
%			
%			\red{Note that, the number of states is at most exponential in the size of $N$.}
%		\item 
%			Predicate $\not\prefix$ of arity two.
%			Consider $t_1, t_2 \in \text{Terms}(X, \cdot, \varepsilon)$.
%			Recall that the predicate $t_1 \not\prefix t_2$ is true if
%			$$
%					|\out(t_1)| < |\out(t_2)|
%				\lor
%					\bigvee_{p=1}^{\max\{|\out(t_1)|, |\out(t_2)|\}}
%					\out(t_1)[p] \neq \out(t_2)[p]
%			$$
%			Remark that, the left-hand side can be realise by the length comparison literal.
%			Furthermore, to check the presence of a mismatch between $\out(t_{1})$ and $\out(t_{2})$ is not direct since the path-acceptor take $\pi_1 \conv \ldots \conv \pi_n$ as input word.
%			Then, the PA need to guess the path-variables which contain the mismatch.
%			
%			Let fix $t_i = \pi_{i,1} \dots \pi_{i, m_i}$ and $t_{i, j} = \pi_{i, 1} \dots \pi_{i, j}$ for each $1 \leq j \leq m_i$.
%			We only provide $P_{k_1, k_2}$ a Parikh automaton of two dimensions which accept the convolutions of $n$ paths of $\paths(A)$ such that
%			$$
%				\bigvee_{p_1=1}^{|\pi_{1, k_1}|}
%				\bigvee_{p_2=1}^{|\pi_{2, k_2}|}
%				\bigwedge \begin{cases}
%					|\out(t_{1, k_1-1})| + p_1 = |\out(t_{2, k_2-1})| + p_2
%				\\
%					\out(\pi_{1, k_1})[p_1] \neq \out(t_{2, k_2})[p_2]
%				\end{cases}
%			$$
%			Intuitively, to guess a position of mismatch $P_{k_1, k_2}$ need to compute in the dimension $i$ the length of $\out(t_{i, k_i-1})$ plus a position of $\pi_{i, k_i}$.
%			So, all data transition $(v_1, \dots, v_n)$ taken by $P_{k_1, k_2}$, the dimension $i$ is increasing with $\sum_{j=1}^{n} |v_j| \times |t_{i, k_i-1}|_j$ where $|t_{i, k_i-1}|_j$ is the number of occurrences of $\pi_j$ in $t_{i, k_i-1}$.
%			In the following, we only describe the case where $p_1 < p_2$ in the above formula but the others cases are dual.
%			The PA $P_{k_1, k_2}$ start in a non-final state where it counts the number of output letters data by data as for the length comparison predicate.
%			To change its state, $P_{k_1, k_2}$ need to non-deterministically guess $d_1$ a data of $\pi_{1, k_1}$ which contain the guessed mismatching of $t_1$.
%			Then, $P_{k_1, k_2}$ goes to an other non-final state which memorise data $d_1$ and a position $p'_1$ such that $1 \leq p'_1 \leq |d_1|$.
%			The value of $p'_1$ is also added in the dimension $1$.
%			Now, $P_{k_1, k_2}$ keep counts the number of output letters but ignore data of $\pi_{1, k_1}$.
%			To reach a final state, $P_{k_1, k_2}$ need to non-deterministically guess $d_2$ a data of $\pi_{2, k_2}$ which contain the guessed mismatching of $t_2$.
%			Then, $P_{k_1, k_2}$ goes to a final state which memorise data $d_1, d_2$ and a positions $p'_1, p'_2$ such that $1 \leq p'_\ell \leq |d_\ell|$.
%			The value of $p'_2$ is also added in the dimension $2$.
%			Finally, $P_{k_1, k_2}$ keep counts the number of output letters but ignore data of $\pi_{1, k_1}$ and $\pi_{2, k_2}$.
%			We conclude by defining $P_{\not\prefix}$ as $P_{<} \cup \bigcup_{k_1 = 1}^{m_1}\bigcup_{k_2=1}^{m_2} P_{k_1, k_2}$.
%			Moreover, we not need to define the negation of this predicate since it can only appear under positive number of negation.
%			
%			Note that, the number of states and dimensions of each $P_{k_1, k_2}$ and $P_{<}$ is constant.
%			So, due to the $m_1 + m_2$ unions $P_{\not\prefix}$ have a number of states and dimensions $O(\sum_{i=1}^{2}|t_i|)$.
%			The maximal absolute value appearing in vectors is $O(\log(\ell) \times \max_{i=1}^{2}|t_i|)$ where $\ell$ is the of the maximal length of output string in $D_f$ and $|t_i| = \sum_{j=1}^{n}|t_i|_j$.
%			We deduce that, the number of different vector is $O((\ell \times \max_{i=1}^{2}|t_i|)^2)$.
%		\end{itemize}
%	\end{enumerate}
%\end{proof}





\subsection{Model-Checking Algorithm -- Proof of
  Theorem~\ref{thm:maintrans}}


\begin{proof}
	We only show the upper bounds since lower bounds come from
        Theorem~\ref{thm:mainNFA}.
	Let set $\psi \in \logic_{\text{Trans}}$ a pattern formula and
        $A$ a transducer. This formula can be put in negation normal
        form in linear time, and we obtain a formula of
        $\logic^+(\O_\trans)$. According to Lemma~\ref{lem:goodtrans}
        and Theorem~\ref{thm:algo}, the model-checking of formulas in
        $\logic^+(\O_\trans)$ is decidable. As for the NFA logic, we
        cannot construct an acceptor for the formula explicitly to get
        our upper bounds. 

        
        The beginning of our PSpace algorithm is the same as for
        NFA. In particular, after a series of transformations
        (negation normal form followed by transformation into path
        formula), we end up with a path formula of
        $\logic^+_P(\O_\trans)$ of the form 
        $\varphi = \bigwedge_{i=1}^{m} r_i \land \bigwedge_{j=1}^{k} s_j$ where each
        $r_i$ are either state, input and path literals and all $s_j$ are
        output literals. 


	We rather presents an algorithm which decides $\varphi \models
        A$ in \textsc{NPSpace} which becomes \textsc{NLogSpace} when
        the formula is fixed. In the following we highlight an upper
        bound on the smallest witness of the non-emptiness of the
        acceptor returned by \texttt{buildAcceptor} and base non it,
        give an \textsc{NPSpace} algorithm which decides if there
        exists such a witness.

	
	We start by considering w.l.o.g a special form of the pattern formula $\varphi$ constructed by Algorithm~\ref{algoG} at line 16.
	We can remove all disjunctions of $\varphi$ in \textsc{NPSpace} by rewriting any sub-formula $\varphi_1 \lor \varphi_2$ by $\varphi_i$ where $i$ is non-deterministically chosen.
	We obtain $\varphi$ of the form $\bigwedge_{i=1}^{m} r_i \land \bigwedge_{j=1}^{k} s_j$ where each $r_i$ are non-output literals and each $s_j$ are output literals.
	Thus, the function \texttt{buildAcceptor} realise only product of PAs, due to the conjunctive form of $\varphi$.
	So, at line 19 the algorithm decides if $\bigcap_{i=1}^{m} L(B_i) \cap \bigcap_{j=1}^{k} L(P_j) \neq \varnothing$ where
		each $B_i$ is an NFA, constructed whether at line 4 using using Lemma~\ref{lem:basic} and
		each $P_j$ is a PA constructed at line 2 using Lemma~\ref{lem:goodtrans}.
	In the following, each $B_i$ are seen as PAs with dimension zero.
	
	Now, we give an \textsc{NPSpace} algorithm which decides the non-emptiness of the product.
	Let denote $d_j, \alpha_j$ and $\ell_j$ the dimension, the number of different vectors occurring on transitions and the maximal absolute value appearing in vectors of $P_j$.
	We define also, $d = \sum_{j=1}^{k} d_j$, $\alpha = \sum_{j=1}^{k} \alpha_j$, $\ell = \max_{j = 1}^{k} \ell_j$ and $s = \prod_{j=1}^{k}\dim(P_j) \times \prod_{i=1}^{m}\dim(B_i)$.
	With Lemma~\ref{lem:witness}, we can ensure that the size of a smallest witness for the non-emptiness is at most exponential in $d, \alpha$ and polynomial in $\ell, s$.
        Calling the function \texttt{buildAcceptor} of
        Algorithm~\ref{algoG} on $\varphi$ returns a Parikh automaton
        which is the product of NFA $B_i$ (for the literals $r_i$) and
        PA $P_j$ (for the constraints $s_j$). The size analysis of
        those automata given in Lemma~\ref{lem:goodtrans} allows us to
        conclude that this product has size $s =
        \prod_{j=1}^{k}\dim(P_j) \times \prod_{i=1}^{m}\dim(B_i)$ such
        that $s\in O(|A|^{|\varphi|})$, where $A$ is the transducer
          being model-checked. Moreover, 	let denote $d_j,
          \alpha_j$ and $\ell_j$ the dimension, the number of
          different vectors occurring on transitions and the maximal
          absolute value appearing in vectors of $P_j$. 
	We define also, $d = \sum_{j=1}^{k} d_j$, $\alpha = \sum_{j=1}^{k} \alpha_j$, $\ell = \max_{j = 1}^{k} \ell_j$.
	Thanks to Lemma~\ref{lem:witness}, we can ensure that the size
        of a smallest witness for the non-emptiness of the product of
        the $B_i$s and the $P_j$s is at most exponential in $d, \alpha$ and polynomial in $\ell, s$.
	By Lemma~\ref{lem:goodtrans}, $d$ is $O(|\varphi|)$ and $\alpha,\ell$ are $O(\log(|A|) \times |\varphi|)$.
	Furthermore, $s$ is $O(|A|^{|\varphi|})$.
	Thus, the size of a smallest witness is $O(|A|^{|\varphi|})$.

        
        Similarly as for the model-checking of the NFA logic, our
        \textsc{NPSpace} (hence \textsc{PSpace}) algorithm guesses
        such a short witness, the transitions of the product of the
        $B_i$ and $P_j$ can be triggered on-the-fly using only
        polynomial space. 	At termination, the algorithm accepts
        if all state variables of the algorithm are assigned to
        accepting states and the Presburger formulas for the
        acceptance condition of each PAs are satisfied.
	Since those formulas are constant (by
        Lemma~\ref{lem:goodtrans}), their satisfiability by
        the counter values can
        be decided in constant space by Theorem~6~(A) of
        \cite{scarpellini}.



        When the formula is fixed, the product of the $B_i$ and $P_j$
        yields a Parikh automaton of polynomial size, with a constant
        Presburger formula and a constant dimension. Moreover, the
        counter values are incremented by natural numbers which are in
        unary, since they correspond to lengths of output words
        occurring on the transitions of the transducer $A$. As a
        result, Theorem~\ref{thm:parikh} tells us that non-emptiness
        can be checked in \textsc{NLogSpace}. \qed
\end{proof}




\subsection{Proof of Theorem~\ref{thm:proptrans}}

In this proof we may ignore variables on arrows when we are not
interested in capturing their values. 
The twinning property has already been expressed in
$\logic_\trans$. We here give a graphical view of the pattern that
characterize it in Figure~\ref{fig:Twinning}.
\begin{figure}
	\centering
	\drawTwinning
	\caption{Pattern of the twinning property.}
	\label{fig:Twinning}
\end{figure}

By \cite{DBLP:conf/fossacs/DaviaudJRV17}, a transducer is
$k$-sequential if and only if it does not satisfy the following
formula (whose pattern is graphically represented in Figure~\ref{fig:BTP}):$$
\begin{array}{l}
\exists_{i = 1}^{k} \exists_{j=0}^{k} \pi_{i,j} \colon q_{i-1, j} \xrightarrow{u_{i, j} \mid v_{i, j}} q_{i, j},\\
\exists_{i = 1}^{k} \exists_{j=0}^{k} \pi'_{i,j} \colon q_{i, j} \xrightarrow{u'_{i, j} \mid v'_{i, j}} q_{i, j},\\
\qquad \bigwedge_{j \neq j'} \bigvee_{i = 1}^{k} \bigwedge_{i' = 1}^{i} \bigwedge
\begin{cases}
u_{i', j} = u_{i', j'} \\
u'_{i', j} = u'_{i', j'} \\
\text{SDel}_{\neq}(
v_{1, j} \dots  v_{i, j},
v'_{i, j},
v_{1, j'} \dots  v_{i, j'},
v'_{i, j'}
)
\end{cases}
\end{array}
$$
\begin{figure}
	\centering
	\drawBTP
	\caption{Pattern of the branching twinning property of order $k$}
	\label{fig:BTP}
\end{figure}



By \cite{DBLP:journals/ijfcs/JeckerF18,ChoffrutDecomposition}, a transducer is
multi-sequential if and only if it is $k$-sequential for some $k$, iff
it does not satisfy the pattern of Figure~\ref{fig:WeakTwinning} where
$\text{SDel}(v_1,v'_1,v_2,v'_2)$ (called the fork property). This pattern is expressed in $\logic_\trans$ by:
$$
\begin{array}{l}
\exists \pi_{0, 1} \colon q_0 \xrightarrow{\phantom{u_1 \mid v_1}} q_1, \\
\exists \pi_{1, 1} \colon q_1 \xrightarrow{u_1 \mid v_1 } q_1, \\
\exists \pi'_{1, 1} \colon q_1 \xrightarrow{u_2 \mid v_2} q_1, \\
\exists \pi_{1, 2} \colon q_1 \xrightarrow{u_1 \mid v'_1} q_2, \\
\exists \pi_{2, 2} \colon q_2 \xrightarrow{u_2 \mid v'_2} q_2, \\
\exists \pi_{2, 3} \colon q_2 \xrightarrow{\phantom{u_1 \mid v_1}} q_3, \\
\end{array}
\bigwedge
\begin{array}{l}
\init(q_0) \\
\final(q_3) \\
\text{SDel}_{\neq}{(v_1, v'_1, v_2, v'_2)}
\end{array} 
$$
\begin{figure}
	\centering
	\drawWeakTwinning
	\caption{Pattern of the fork property}
	\label{fig:WeakTwinning}
\end{figure}


By \cite{DBLP:conf/mfcs/SakarovitchS08,DBLP:journals/acta/Weber89},
a transducer is finite valued if and only if it is $k$-valued for some
$k$, iff it does not satisfy any of the following patterns:
\begin{itemize}
	\item Figure~\ref{fig:CoTerminalCircuits} where $v_1 \neq v_2$ expressed in $\logic_\trans$ by:
	$$
	\begin{array}{l}
	\exists \pi_{0, 1} \colon q_0 \xrightarrow{\phantom{u \mid v_1}} q_1, \\
	\exists \pi_{1, 1} \colon q_1 \xrightarrow{u \mid v_1 } q_1, \\
	\exists \pi_{1, 3} \colon q_1 \xrightarrow{\phantom{u \mid v_1}} q_3, \\
	\exists \pi_{0, 2} \colon q_0 \xrightarrow{\phantom{u \mid v_1}} q_2, \\
	\exists \pi_{2, 2} \colon q_2 \xrightarrow{u \mid v_2} q_2, \\
	\exists \pi_{2, 3} \colon q_2 \xrightarrow{\phantom{u \mid v_1}} q_3,
	\end{array}
	\bigwedge
	\begin{cases}
	\init(q_0) \\
	\final(q_3) \\
	v_1 \neq v_2
	\end{cases} 
	$$
	\begin{figure}
		\centering
		\drawCoTerminalCircuits
		\caption{Pattern of co-terminal circuits}
		\label{fig:CoTerminalCircuits}
	\end{figure}
	\item Figure~\ref{fig:Dumbbell} where $s_1 \neq s_2$ and $v_1v_2 \neq v_2v_3$ expressed in $\logic_\trans$ by:
	$$
	\begin{array}{l}
	\exists \pi_{0, 1} \colon s_0 \xrightarrow{\phantom{u \mid v_1}} s_1, \\
	\exists \pi_{1, 1} \colon s_1 \xrightarrow{u \mid v_1 } s_1, \\
	\exists \pi_{1, 2} \colon s_1 \xrightarrow{u \mid v_2} s_2, \\
	\exists \pi_{2, 2} \colon s_2 \xrightarrow{u \mid v_3} s_2, \\
	\exists \pi_{2, 3} \colon s_2 \xrightarrow{\phantom{u \mid v_1}} s_3,
	\end{array}
	\bigwedge
	\begin{cases}
	\init(s_0) \\
	\final(s_3) \\
	s_1 \neq s_2\\
	v_1v_2 \neq v_2v_3
	\end{cases} 
	$$
	\begin{figure}
		\centering
		\drawDumbbell
		\caption{Pattern of the dumbbell computation}
		\label{fig:Dumbbell}
	\end{figure}
	\item Figure~\ref{fig:W} where $|v_1| \neq |v_2|$  expressed in $\logic_\trans$ by:
	$$
	\begin{array}{l}
	\exists \pi_{0, 1} \colon r_0 \xrightarrow{\phantom{u_1 \mid v_1}} r_1, \\
	\exists \pi_{1, 1} \colon r_1 \xrightarrow{u_1 \mid v_1 } r_2, \\
	\exists \pi_{2, 2} \colon r_2 \xrightarrow{u_2\phantom{\mid v_1}} r_2, \\
	\exists \pi_{2, 2} \colon r_2 \xrightarrow{u_3\phantom{\mid v_1}} r_1, \\
	\exists \pi_{1, 1} \colon r_1 \xrightarrow{u_1\phantom{\mid v_1}} r_3, \\
	\exists \pi_{3, 1} \colon r_3 \xrightarrow{u_2 \mid v_2} r_3, \\
	\exists \pi_{3, 2} \colon r_3 \xrightarrow{u_3\phantom{\mid v_1}} r_4, \\
	\exists \pi_{4, 2} \colon r_4 \xrightarrow{u_1\phantom{\mid v_1}} r_5, \\
	\exists \pi_{5, 1} \colon r_5 \xrightarrow{u_2\phantom{\mid v_1}} r_5, \\
	\exists \pi_{5, 1} \colon r_5 \xrightarrow{u_3\phantom{\mid v_1}} r_4, \\
	\exists \pi_{4, 2} \colon r_4 \xrightarrow{\phantom{u_1 \mid v_1}} r_6,
	\end{array}
	\bigwedge
	\begin{cases}
	\init(r_0) \\
	\final(r_6) \\
	|v_1| \neq |v_2|
	\end{cases} 
	$$
	\begin{figure}
		\centering
		\drawW
		\caption{Pattern of the W computation}
		\label{fig:W}
	\end{figure}
\end{itemize}


==> generic.tex <==

\begin{theorem}
	If there exists an effectively good class of path tuple acceptors for a monoid $\M$ and a set of output predicates $\O$, then the model-checking problem for any automata with output over $\M$ and a pattern formula over $\O$ is decidable by Algorithm~\ref{algoG}.
\end{theorem}


\begin{algorithm}\caption{Generic Model-Checking}\label{algoG}
		\DontPrintSemicolon
		\SetKwInput{In}{Inputs}
		\SetKwInput{Out}{Output}
		\SetKwFunction{acceptor}{buildAcceptor}
		\SetKwFunction{match}{patternMatching}
		\SetKwProg{funacceptor}{Functor}{$\colon \C|_n$}{end}
		\SetKwProg{funmatch}{Functor}{$\colon \bool$}{}
		\SetKw{with}{with}
		\SetKw{bool}{boolean}
		
		\In{\text{}
			\\\quad\ A pattern formula $\psi$ in negative normal form
			\\\quad\ An automaton $A$ over $\Lambda$ with output over $\M$
		}
		\Out{Decide $T \models \psi$}
		\KwData{\text{}
			\\\quad\ The natural $n$ refer $|\Var(\psi)|$
			\\\quad\ The class of path acceptors $\C$ is effectivily good for $\M$ with $\O$.
		}
		\BlankLine
		
		\funacceptor{\acceptor{$\varphi \colon \logic(\O)$}}{
			\ShowLn
			\uIf{$\varphi \equiv l$ \with $l$ an output literal}{
				\Return{$M_{l, n}$}\;
				%\tcc*[l]{by item \ref{goodout} of the good class definition}
			}
			\ShowLn
			\uIf{$\varphi \equiv l$ \with $l$ a non-output literal}{
				\Return{$M_{l, n}$}\;
				%\tcc*[l]{by Lemma~\ref{lem:logicREG} and item \ref{goodreg} of the good class definition}
			}
			\ShowLn
			\uIf{$\varphi \equiv \varphi_1 \lor \varphi_2$ }{
				$M_1 \colon \C|_n \affect \acceptor{$\varphi_1$}$\;
				$M_2 \colon \C|_n \affect \acceptor{$\varphi_2$}$\;
				\Return{$M_1 \cup M_2$}\;
				%\tcc*[l]{by item \ref{goodclos} of the good class definition}
			}
			\ShowLn
			\If{$\varphi \equiv \varphi_1 \land \varphi_2$}{
				$M_1 \colon \C|_n \affect \acceptor{$\varphi_1$}$\;
				$M_2 \colon \C|_n \affect \acceptor{$\varphi_2$}$\;
				\Return{$M_1 \cap M_2$}\;
				%\tcc*[l]{by item \ref{goodclos} of the good class definition}
			}
		}
		\BlankLine

		\funmatch{\match{$A \colon \trs(\Lambda, \M), \psi \colon \logic(\O)$}}{
			\ShowLn
			$M_P \colon \C|_n \affect \paths(A)^{n}$\;
			%\tcc*[l]{by Lemma~\ref{lem:pathsREG} and item \ref{goodreg} of the good class definition}
			\ShowLn
			$M \colon \C|_n \affect \acceptor{$\psi$} \cap M_P$\;
			%\tcc*[l]{by items \ref{goodclos} of the good class definition}
			\ShowLn
			\Return{$\sem{M} \neq \varnothing$}\;
			%\tcc*[l]{since $\C$ is an effective good class}
		}
\end{algorithm}
\begin{proof}
	We can assume w.l.o.g that $\varphi$ is in negative normal form i.e negation operator is only apply on atoms, otherwise we rewrite the formula in linear time using De Morgan's laws.
	
	First, we show the correctness of \textsf{buildAcceptor} of Algorithm~\ref{algoG}.
	We claim that \textsf{buildAcceptor} with $n$ and $\C$ is a function which take a pattern formula $\varphi$ in negative normal form and return a machine $M \in \C|_n$ such that $\sem{\varphi}_A = \paths(A)^{n} \cap \sem{M}$.
	The proof goes by structural induction on $\varphi$.
	\begin{enumerate}
		\item[2.]
			At this line, $\varphi$ is of the form $p(t_1, \dots, t_{\alpha(t)})$ or $\lnot p(t_1, \dots, t_{\alpha(t)})$.
			Using the item \ref{goodout} of the good class definition, we can construct $M, M' \in \C|_n$ such that 
			$$
			\begin{array}{ll}
			\sem{M} = \left\{ \begin{array}{c|c}
			\left( \nu(\pi_1), \dots, \nu(\pi_n) \right)
			&
			\nu \colon X\rightarrow \paths(\Lambda, Q, D) \land
			(t^{\nu, \M}_1, \dots, t^{\nu, \M}_{\alpha(p)}) \in \sem{p}_A
			\end{array}\right\}
			\smallskip\\
			\sem{M'} = \left\{\begin{array}{c|c}
			\left( \nu(\pi_1), \dots, \nu(\pi_n) \right)
			&
			\nu \colon X\rightarrow \paths(\Lambda, Q, D) \land
			(t^{\nu, \M}_1, \dots, t^{\nu, \M}_{\alpha(p)}) \notin \sem{p}_A
			\end{array}\right\}
			\end{array}
			$$
		\item[4.]
			At this line, $\varphi$ does not contain output predicates.
			So, by Lemma~\ref{lem:logicREG}, there exists effectively a regular set of $n$-path tuples $R$ such that $\sem{\varphi}_A = \paths(A)^{n} \cap R$.
			Using the item \ref{goodreg} of the good class definition, we can construct $M \in \C|_n$ such that $\sem{M} = R$.
		\item[6.]
			At this line, $\varphi$ is of the form $\varphi_1 \lor \varphi_2$.
			For $1 \leq i \leq 2$, by induction hypothesis applied on $\varphi_i$, we can construct $M_i$ such that $\sem{\varphi_i}_A = \paths(A)^{n} \cap \sem{M_i}$.
			Using the item \ref{goodclos} of the good class definition, there exists effectively a machine $M \in \C|_n$ such that $\sem{M} = \sem{M_1} \cup \sem{M_2}$.
			$$
				\begin{array}{ll}
					\sem{\varphi}_A &= \sem{\varphi_1}_A \cup \sem{\varphi_2}_A
				\\
					&=
						\left( \paths(A)^{n} \cap \sem{M_1} \right)
						\cup
						\left( \paths(A)^{n} \cap \sem{M_2} \right)
				\\
					&= \paths(A)^{n} \cap \left( \sem{M_1} \cup \sem{M_2} \right)
				\end{array}
			$$
		\item[10.]
			This line is the dual of above.
	\end{enumerate}

	Now, we show the correctness of \textsf{patternMaching} of Algorithm~\ref{algoG}.
	%We claim that \textsf{patternMaching} with $n$ and $\C$ is a function which take a pattern formula $\varphi$ in negative normal form, an automaton $A$ over $\Lambda$ with output over $\M$ and decide $A \models \varphi$.
	At line~15, we construct the machine $M_P$.
	By Lemma~\ref{lem:pathsREG} there exists effectively a NFA $B$ such that $L(B) = \paths(A)$.
	Using the item \ref{goodreg} of the good class definition, we can construct a machine $M_P \in \C|_n$ such that $\sem{M_P} = \left(L(B)^n\right)^\sharp = \paths(A)^n$.
	At line~16 we construct the machine $M$.
	By the claim \textsf{buildAcceptor} return a machine $M' \in \C|_n$ such that $\sem{\psi}_A = \paths(A)^{n} \cap \sem{M'}$.
	Using the item \ref{goodclos} of the good class definition, we can construct a machine $M \in \C|_n$ such that $\sem{M} = \sem{M_P} \cap \sem{M'} = \sem{\psi}_A$.
	Finally, at line~17 we have $\sem{M} \neq \varnothing$ if and only if $\sem{\psi} \neq \varnothing$.
	In addition, by the definition of good class, $\sem{M} \neq \varnothing$ is decidable.
	\qed
\end{proof}



